Revenue Sharing in the Internet: A Moral Hazard Approach and a Net-neutrality Perspective

Revenue sharing contracts between Content Providers (CPs) and Internet Service Providers (ISPs) can act as leverage for enhancing the infrastructure of the Internet. ISPs can be incentivized to make investments in network infrastructure that improve Quality of Service (QoS) for users if attractive contracts are negotiated between them and CPs. The idea here is that part of the net profit gained by CPs are given to ISPs to invest in the network. The Moral Hazard economic framework is used to model such an interaction, in which a principal determines a contract, and an agent reacts by adapting her effort. In our setting, several competitive CPs interact through one common ISP. Two cases are studied: (i) the ISP differentiates between the CPs and makes a (potentially) different investment to improve the QoS of each CP, and (ii) the ISP does not differentiate between CPs and makes a common investment for both. The last scenario can be viewed as \emph{network neutral behavior} on the part of the ISP. We analyse the optimal contracts and show that the CP that can better monetize its demand always prefers the non-neutral regime. Interestingly, ISP revenue, as well as social utility, are also found to be higher under the non-neutral regime.

==> GeneralCase.tex <==
%\section{Comparison between neutral and non-neutral regime}In numerical comparisons we fix $r_2$ and
$c$ and vary $r_1$.
\subsubsection{\textbf{Contracts}}
The following proposition provides a comparison of the equilibrium
contracts in both the regimes.

\begin{figure*}[!t]
	\centering
	\subfloat[]{\includegraphics[scale=0.05]{figures/betascatter}\label{fig:betascatter}}
			\hspace{0.4cm}
	\subfloat[]{\includegraphics[scale=0.3]{figures/beta1a}
		\label{fig:beta1a}}
	\hspace{0.4cm}
	\subfloat[]{\includegraphics[scale=0.3]{figures/beta1e}
		\label{fig:beta1e}}
	\vspace{-.3cm}
	\caption {(\ref{fig:betascatter}) gives scatter-plot of $\beta$s. (\ref{fig:beta1a}) and (\ref{fig:beta1e}) gives variation of equilibrium $\beta_1$ vs $r_1$ under neutral and non-neutral regime.}
	\label{fig:beta}
\end{figure*}

\begin{figure*}[!h]
	\centering
	
	\subfloat[]{\includegraphics[scale=0.3]{figures/CPutilityscatter}		\label{fig:CPutilityscatter}}
	\hspace{0.4cm}
	\subfloat[]{\includegraphics[scale=0.3]{figures/CP1utility}\label{fig:CP1utility}}
	\hspace{0.4cm}
	\subfloat[]{\includegraphics[scale=0.3]{figures/CP2utility}\label{fig:CP2utility}}
	\vspace{-.3cm}
	\caption {(\ref{fig:CPutilityscatter}) shows scatterplot for the CP utilities at equilibrium. (\ref{fig:CP1utility})\&(\ref{fig:CP2utility}) compare $\mbox{CP}_1$ utility in both regimes as $r_1$ varies.}
	\label{fig:CPUtility}
\end{figure*}


 
 \begin{proposition} 
 	\label{prop:contracts}
 	Fix $r_2 > 0.$ We have
 	\begin{itemize}
 		\item For $r_1\geq r_2$, $\beta_2^{NN} \geq \beta_2^{N}$.  $\beta_2^{N}$ decreases in $r_1$.
 		\item  For $r_1\geq r_1^*$, $\beta_1^{N}>\beta_1^{NN}$.  $\beta_1^{N}$ decreases in $r_1$ for $r_1>r_1^*$. 
 	\end{itemize}	
 \end{proposition}
 
Fig. (\ref{fig:betascatter}) shows behavior of $\beta_i, i=1,2$ in the
non-neutral and neutral regime. When $r_1 \geq >r_2$, the non-dominant
CP shares a higher fraction of its revenue in the non-neutral
regime. This region is colored red and green. However the same is true
for the dominant CP only in the region colored red. The dominant CP
share a higher fraction of its revenue in neutral regime in the region
colored green.

While both $\beta_1^{NN}$ and $\beta_2^{NN}$ are non-increasing as
seen from Thm.~\ref{Thm:NN-asy}, only $\beta_2^{N}$ is non-increasing
in $r_1$. $\beta_1^{N}$ is non-increasing only in the region $r_1\geq
r_1^*$ and it may be increasing or decreasing in $r_1$ satisfying
$r_1<r_1^*$ as shown in Figs. (\ref{fig:beta1a}) and
(\ref{fig:beta1e}). Due to this behavior of $\beta_1^{N}$, it is not
always the case that the dominant CP contributes a higher revenue
share to the ISP in the neutral regime for $r_1 < r_1^*;$ however,
this is always the case for $r_1 \geq r_1^*$ as shown in
Prop.~\ref{prop:contracts}.

In the black colored region where $r_i/c < 1, i=1,2$ none of the CPs
share anything in both the regimes, i.e., $\beta_i^N=\beta_i^{NN}=0$
for all $i=1,2$. The yellow colored region $1<r_i/c <2, i=1,2$, where
CPs revenue share is positive in the non-neutral regime and it is zero
in the neutral regime. %Hence $\beta_i^{N}>\beta_i^{NN}$ for $i=1,2$.

\subsubsection{\textbf{Utility of CPs}}
In this subsection we compare the utilities of the CPs in both the
regimes. The following proposition characterizes preference of the CPs
for the neutral and non-neutral regime.
%\begin{figure}[h!] \label{fig:CPutility}
%	\centering
%	{\includegraphics[scale=0.3]{figures/CP1utility}%
%	}
%	{\includegraphics[scale=0.3]{figures/CP2utility}%
%	}
%	\caption {Comparison of CP's utility between Non-neutral and neutral when CPs are asymmetric. We fix $c=1, r_2=2$ and vary $r_1$ from 2 to 30.}
%	\label{fig:comparison}
%\end{figure}
%
%\begin{figure}[h] \label{fig:CPUscatter}
%	\centering
%	\includegraphics[scale=0.3]{figures/CPutilityscatter}
%	\caption{Scatter plot for comparison of utility of $CP_i; i=1,2$ between non-neutral and neutral regime over different range of $r_i/c$}
%\end{figure}



\begin{proposition}
\label{prop:CPUtility}
Fix an $r_2$. We have
\begin{itemize}
	\item For all $r_1>r_2$, the dominant CP prefers the non-neutral regime.
	\item For all $r_1\geq r_1^*$,  the non dominant CP prefers the neutral regime.
\end{itemize}
\end{proposition}

Figure \ref{fig:CPUtility} shows the scatter plot utilities of the
players in both the regimes. For $r_1\geq >r_2$, the dominant CP has
higher utility in the non-neutral regime as can be observed from the
red and magenta regions. This is because in the neutral regime, the
dominant CP is `forced' to pay for capacity investment that benefits
the non-dominant CP. Indeed, note that in the region $r_1\geq r_1^*$,
the dominant CP shares a smaller fraction of its revenue in the
non-neutral regime, but still ends-up with a higher utility. In this
region, the non-dominant CP obtains higher utility in the neutral
regime (thanks to the `subsidization' from the dominant CP) and hence
prefers it. However for the region $r_1< r_2^*$ the non-dominant CP may or may not prefer the neutral regime depending on the value
of $r_2$ as shown in Figs.~(\ref{fig:CP1utility}) and
(\ref{fig:CP2utility}).
% as the asymmetry between CPs increases,the CP with higher revenue per click rate (CP$_1$) continue higher utility in the non-neutral regime, however, CP with lower revenue per click rate (CP$_2$) becomes better off in the neutral regime after certain small value of $r_1$ for every fixed $r_2$. 


\subsubsection{\textbf{Utility of ISP}}
We next compare utility of the ISP in the non-neutral and neutral
regime. For simplicity, we take ISP utility to be the expected revenue
given as $\UISP=\mathbb{E}[\sum_{i} s(X_i)-ca_i]$ (ignoring the
risk-sensitive utility defined before). Its value in the non-neutral
regime is given by:
\[\UISP^{NN}=(1-2\beta_1^{NN})r_1+(1-2\beta_2^{NN})r_2+2c,\]
and in the neutral regime for all $r_1\geq r_1^*$ is given by:
\[\UISP^{N}=(1-2\beta_1^{N})r_1+2c.\] 
The utility for  $r_1< r_1^*$ in the neutral regime is cumbersome and we skip its expression. The following lemma demonstrates the ISPs earnings are higher in the non-neutral regime for monetization power of the dominant CP is much larger than the other, i.e., $r_1$ is much larger than $r_2$.
\begin{lemma} \label{lma:ISPutilitycomp}
	There exist $r_1^b>r_1^*$, such that for all $r_1>r_1^b$ ISP
        has better utility in the non-neutral regime.
\end{lemma}

Comparison of the ISP utilities in general is not analytically
tractable. We thus plot it under neutral and non-neutral regime in
Fig.~ \ref{fig:ISPUtility}. As seen in the first figure, ISP for a
fixed $r_2$ and $c$, for all $r_1$ utility of ISP in the non-neutral
regime is higher than in the. Also, we can observe the same behavior
is the scatter plot given in the second figure.
%neutral one. That is for all $r_1\geq r_2$ ISP is better off  in non-neutral regime than in neutral. Same analysis is true for the case where $r_2>r_1$, and thus, ISP is always better off in non-neutral regime. Figure \ref{fig:ISPscatterplot} also shows that ISP is always better off in non-neutral regime.


\begin{figure}[h!]
	\centering
	{\includegraphics[scale=0.29]{figures/ISPutility}%
	}
	{\includegraphics[scale=0.29]{figures/ISPutilityscatter}%
	}
	\caption {Comparison of ISP utility between Non-neutral $c=1, r_2=2$ and scatter plot. }
	\label{fig:ISPUtility}
\end{figure}

\subsubsection{\textbf{Social Utility}}
Finally, we compare social utility in both the regimes. In the non-neutral regime, social utility is given by
\begin{align*}
SU^{NN}=&U_{CP_1}^{NN}+U_{CP_1}^{NN}+U_{ISP}^{NN}\\
=&r_1\log\left(\frac{\beta_1^{NN}r_1}{c}\right)+r_2\log\left(\frac{\beta_2^{NN}r_2}{c}\right)-(\beta_1^{NN}r_1+\beta_2^{NN}r_2)+2c.
\end{align*} 
Similarly, social utility in the neutral case is given as
\begin{align*}
&SU^N=U_{CP_1}^N+U_{CP_1}^N+U_{ISP}^N\\
&=(r_1+r_2)\log\left(\frac{\beta_1^Nr_1+\beta_2^Nr_2}{c}\right)-(\beta_1^Nr_1+\beta_2^Nr_2)+2c.
\end{align*} 
\begin{figure}[h!] \label{fig:SocialUtility}
	\centering
	{\includegraphics[scale=0.29]{figures/SU}%
	}
	{\includegraphics[scale=0.29]{figures/SUscatter}%
	}
	\caption {Comparison of social utility between neutral and non-neutral regime for $c=1, r_2=2$ and scatter plot. }
\end{figure}
As it is not easy to compare the social utilities analytically, we do numerical comparison in the first part of Fig.5. As seen social utility in the non-neutral regime dominates that in the neutral regime for all values of $r_1$ for a given $r_2$ and $c$. The scatter plot in the second part of the figure also gives the same observation.
\subsubsection{\textbf{Total Effort by ISP}}
In this section, we compare the total effort by ISP for CPs in the non-neutral and neutral regime. We focus on the region where $r_1>r_1^*$. Total effort in non-neutral for all $r_1$ regime is given by
\begin{align*}
	A^{NN}&=a_1^{NN}+a_2^{NN}=\frac{\beta_1^{NN}r_1}{c}-1+\frac{\beta_2^{NN}r_2}{c}-1\\
	&=\frac{\frac{r_1}{c}}{W(\frac{r_1}{c}e)}+\frac{\frac{r_2}{c}}{W(\frac{r_2}{c}e)}-2
\end{align*}
Similarly, total effort in neutral regime is
\begin{align*}
	A^{N}=2a^{N}=2\left(\frac{\beta_1^{N}r_1}{2c}-1\right)=\frac{\frac{r_1}{c}}{W(\frac{r_1}{2c}e)}-2 \hspace{.75mm}\forall \hspace{.75mm}r_1>r_1^*
\end{align*}
\begin{figure}[!t] \label{fig:TotalEffort}
	\centering
	{\includegraphics[scale=0.29]{figures/totaleffort}%
	}
	{\includegraphics[scale=0.35]{figures/totaleffortscatter}%
	}
	\caption{Scatter plot for comparison between total effort (investment) by ISP in non-neutral and neutral regime over different range of $r_i/c$}
\end{figure}
\begin{lemma} \label{lma:totaleffortcomp}
	There exist some $r_1^a$ sufficiently larger than $r_1^*$, s.t. for all $r_1^a>r_1^*$, total effort by ISP is higher in neutral regime than in the  non-neutral.
\end{lemma}
The threshold $r_1^a$ is given by following equation:
$$r_1^a \left(\frac{1}{W(\frac{r_1^a}{2c}e)}-\frac{1}{W(\frac{r_1^a}{c}e)}\right)=\frac{{r_2}}{W(\frac{r_2}{c}e)}$$
It can be seen from above equation that $r_1^a$ is monotonically increasing in $r_2$.\\

The above lemma implies that total effort by ISP in the neutral regime becomes higher when there is high asymmetry between CP's revenue per click rates. 

==> Journal Version Arxiv/AsymmetricCase.tex <==
In this section we study the asymmetric case where monetizing power of all the CPs need not be the same, i.e., $r_i\neq r_j$ for $i\neq j$.
Our interest in this section is to understand how disparity in the
monetizing power influences preference of the players for the neutral
and non-neutral regimes. We focus on the case with two
CPs ($n=2$) and without loss of generality assume that monetizing
power of $\mbox{CP}_1$ is more than that of $\mbox{CP}_2,$ i.e., $r_1>r_2.$ We refer to $\mbox{CP}_1$ as dominant and  $\mbox{CP}_2$ as non-dominant.

Recall that the objective of the $CP_i, i\in \mathcal{N}$ in the
non-neutral regime can be expressed as
\begin{equation*}
\max_{\beta_i \in [0,1]} \hspace{2mm} (1-\beta_i)r_i\log\left(\max\left(\frac{\beta_ir_i}{c},1\right)\right),
\end{equation*}
and in the neutral regime it can be expressed as
\begin{equation*}
  \max_{\beta_i \in [0,1]} \hspace{2mm} (1-\beta_i)r_i\log\left(\max\left(\frac{\sum_i\beta_ir_i}{nc},1\right)\right).
\end{equation*} 
As discussed in Section \ref{sec:MultipleSymmetric}, the case
$r_i/c\leq 1$ for all $i \in \mathcal{N}$ is not interesting as none
of the CPs would have the incentive to contribute towards ISP effort.
Thus, in this section, we restrict ourselves to the case where
$r_i/c>1$ for at least one $i \in \mathcal{N}$.  The following results
characterize the equilibrium contracts for the neutral and the
non-neutral regime.\footnote{The characterization of equilibrium
  contracts can actually be done for any $n;$ see Appendix~\ref{app:AsymmetricMultipleCPs}.}

\subsection{Equilibrium contracts}

In the non-neutral regime, the interactions between each CP and the
ISP remain decoupled, and thus the equilibrium contracts follow easily
from Theorem~\ref{thm:equillibrium-NN}.
\begin{cor}
  \label{thm:AsymBetaNN}
  In the non-neutral regime, the equilibrium contract
  $(\beta_1^{NN},\beta_2^{NN})$ is as follows:
  $$\beta_i^{NN} = \begin{cases}
      0  &\mbox{  if }  \frac{r_i}{c} \leq 1, 
      % \\
      % \left(0, \frac{1}{W\left(\frac{r_2}{c}e\right)}\right)  &\mbox{  if }  \frac{r_%1}{c} \le 1, \frac{r_2}{c} > 1, 
      \\
      \frac{1}{W\left(\frac{r_i}{c}e\right)}  &\mbox{  if }  \frac{r_i}{c} > 1.
    \end{cases}$$
\end{cor}
\noindent Note that when $\frac{r_i}{c} \leq 1,$ the equilibrium
contract between $\CPi$ and the ISP is not uniquely defined, since any
$\beta_i \in [0,1]$ would result in zero surplus to $\CPi.$


%Notice that if $r_i$ increases, $\beta_i^*$ decreases, i.e., $\CPi$
% shares a small fraction of its revenue with the ISP.  \textbf{This is
%   because if a CP's capability to translate its demand to earning
%   improves, then it may require less effort from the ISP to improve
%   demand for its content and hence can reduce the incentives it gives
%   through revenue-sharing.}  \mh{need to explain this better} \jk{I
%   think this is essentially a repeat of a result already stated and
%   interpreted in the previous section. So no need to spend much time
%   on this.}


% Similar result for $n>2$ can be computed and is given in the
% appendix.
%\subsection{Non-neutral regime}
%The of each $\CPi, i\in N,$ can be expressed: 
%
%Following arguements similar to Thm.~\ref{thm:equillibrium-NN}, the equilibrium contracts can be given as follows: 

%Equilibrium contract is give as:
%\begin{equation}
%\beta_i^*=\begin{cases}
%\frac{1}{W\left(\frac{r_i}{c}e\right)} &\mbox{  if }  \frac{r_i}{c} >1, \\
%0  &\mbox{  else }  
%\end{cases}
%\end{equation}
%\subsection{Neutral regime}
%The objective function of $\CPi, i\in N$ in the neutral regime can then be expressed as follows:
%\begin{equation*}
%\max_{\beta_i \in [0,1]} \hspace{2mm} (1-\beta_i)r_i\log\left(\max\left(\frac{\sum_i\beta_ir_i}{nc},1\right)\right)
%\end{equation*} 


%We focus on the case of $n=2$ for comparing the non-neutral and
% neutral regime. Without loss of generality, we assume
% $r_1 \geq r_2$, i.e., $\mbox{CP}_1$ earns higher per unit demand
% than $\mbox{CP}_2$. We refer to $\mbox{CP}_1$ as the dominant CP and
% $\mbox{CP}_2$ as the non-dominant CP. \textbf{This constraint will
% be considered for the rest of the paper.} What does this line mean?
% We begin with the non-neutral regime.

%\subsection{Non-neutral regime}
%Under the non-neutral regime, it is easy to see that when
%$\overline{H}=-1$, the CP decisions are no more coupled. The
%optimization problem for $CP_i, i=1,2$ simplifies to:
%\begin{align*}
%&\max_{\beta_i\in [0,1]} \hspace{2mm} (1-\beta_i)r_i\log\left(\max\left(\frac{\beta_ir_i}{c}-1,0\right)+1\right).
%\end{align*}
%Let  $W(\cdot)$ denote the stand LambertW function \textcolor{blue}{\cite{}} taking values on the principle branch. The optimal contract is characterized in term LambertW function in the following. %Each CP has his own constraint optimization problem with common constraint which is the optimization problem of the ISP. Then, the global problem can be seen as a hierarchical non-cooperative game between CPs (here 2 leaders) and one ISP (one follower).Usually, this type of complex game involves the framework of Generalized Nash Equilibrium Point (GNEP) and tools from it mainly for optimization theory and KKT conditions. In our setting, we are able to determine explicitly the equilibrium solution of this hierarchical game between two CPs and one ISP.
%


%\subsection{Neutral Regime}
%In the neutral regime, ISP is forced to make the same investment
%decision for both CPs, i.e., $a_1=a_2=a$. The optimization problem for
%CP $i$ in this case simplifies to:
%\begin{align*}
%&\max_{\beta_i \in [0,1]} \hspace{2mm} (1-\beta_i)\log\left(\max\left(\frac{\beta_1r_1+\beta_2r_2}{2c}-1,0\right)+1\right)r_i.
%\end{align*} 

Next, we characterize equilibrium contract in the neutral regime.
\begin{thm} \label{thm:AsymBetaN} Consider the neutral regime, with
  $r_1 > r_2.$ If $r_1/c \leq 2$ then
  $(\beta_1^N,\beta_2^N)=(0,0)$. If $r_1/c > 2,$ then the equilibrium
  contract is given by:\\ \begin{equation}
    (\beta_1^N,\beta_2^N)=\begin{cases} (\overline{\beta}_1,
      \overline{\beta}_2) &\mbox{ if } \frac{r_1+r_2}{r_1-r_2} >
      2W\left(\frac{r_1+r_2}{4c}\sqrt{e}\right), \\ \left(\frac{1}{
          W\left(\frac{r_1}{2c}e\right)},0\right) &\mbox{
        otherwise}, \end{cases} \label{eqn:NeutralConds} \end{equation}
  where \begin{equation}\nonumber
    \overline{\beta}_1=\frac{r_1+r_2}{4r_1W\left(\frac{r_1+r_2}{4c}\sqrt{e}\right)}-\frac{r_2-r_1}{2r_1},
    \overline{\beta}_2=\frac{r_1+r_2}{4r_2
      W\left(\frac{r_1+r_2}{4c}\sqrt{e}\right)}-\frac{r_1-r_2}{2r_2}.  \end{equation}
\end{thm}
%

When $r_1/c \leq 2,$ the equilibrium contract is not unique, though
the outcome is that ISP effort equals zero. When $r_1/c > 2,$ the
equilibrium contract is unique, and at least one CP (specifically,
$\mbox{CP}_1$) is guaranteed to contribute a constant fraction of her
revenue to the ISP. Note that when $r_1/c \in (1,2],$ there is no CP
contribution in the neutral regime, even though there is in the
non-neutral regime. 

To interpret the equilibrium when $r_1/c > 2,$ let $r_1^*:=r_1^*(r_2)$
denote the value of $r_1$ that satisfies the following relation for a
given $r_2$
$$\frac{r_1+r_2}{r_1-r_2} = 2W\left(\frac{r_1+r_2}{4c}\sqrt{e}\right).$$
For $r_1\leq r_1^*$ the condition in (\ref{eqn:NeutralConds}) holds where revenue shared by both the CPs is strictly positive,
i.e., $\beta_i^{N}>0$ for all $i\in \N$. For $r_1 > r_1^*$ the condition in (\ref{eqn:NeutralConds}) fails
in which only the $\mbox{CP}_1$'s share is strictly
positive and $\mbox{CP}_2$ does not share anything, i.e.,
$\beta_1^N>0$ and $\beta_2^N=0$. Further, it is easy to verify that
$r_1^*$ is monotonically increasing in $r_2$ and $r_1^*> r_2$.

\subsection{Comparison between Neutral and Non-neutral regimes}

Having characterized the equilibrium contracts in both regimes, we
compare and contrast the neutral and non-neutral regimes in the
remainder of this section. We begin by comparing the equilibrium
contracts, followed by CP/ISP utility, social utility, and finally ISP
effort.

% We ae now ready to compare the contracts, utilities of the CPs and
% the ISP, and the social utility at equilibrium obtained under the
% neutral and the non-neutral regime.
\subsubsection{\textbf{Contracts}}
The following proposition provides a comparison of the equilibrium
contracts in both the regimes.

\begin{figure*}[!t]
	\centering
	\subfloat[]{\includegraphics[scale=0.05]{figures/betascatter}\label{fig:betascatter}}
	\hspace{0.4cm}
	\subfloat[]{\includegraphics[scale=0.3]{figures/beta1a}
		\label{fig:beta1a}}
	\hspace{0.4cm}
	\subfloat[]{\includegraphics[scale=0.3]{figures/beta1e}
		\label{fig:beta1e}}
	\caption {Fig.~\ref{fig:betascatter} gives scatter-plot of $\beta$s. Figs.~\ref{fig:beta1a} and \ref{fig:beta1e} shows variation of equilibrium $\beta_1$ vs $r_1$ under neutral and non-neutral regime.}
	\label{fig:beta}
\end{figure*}

\begin{figure*}[!h]
	\centering
	
	\subfloat[]{\includegraphics[scale=0.3]{figures/CPutilityscatter}		\label{fig:CPutilityscatter}}
	\hspace{0.4cm}
	\subfloat[]{\includegraphics[scale=0.3]{figures/CP1utility}\label{fig:CP1utility}}
	\hspace{0.4cm}
	\subfloat[]{\includegraphics[scale=0.3]{figures/CP2utility}\label{fig:CP2utility}}
	\caption {Fig.~\ref{fig:CPutilityscatter} shows scatterplot for the CP utilities at equilibrium. Figs.~(\ref{fig:CP1utility}) \& (\ref{fig:CP2utility}) compare $\mbox{CP}_1$ utility in both regimes as $r_1$ varies.}
	\label{fig:CPUtility}
\end{figure*}



\begin{proposition} 
  \label{prop:contracts}
  Fix $r_2 > 0.$ We have
  \begin{itemize}
  \item For $r_1> r_2$, $\beta_2^{NN} \geq \beta_2^{N}$.
    Moreover, $\beta_2^{N}$ decreases in $r_1$.
  \item For $r_1\geq r_1^*$,
    $\beta_1^{N}>\beta_1^{NN}$. Moreover, $\beta_1^{N}$
    decreases in $r_1$ for $r_1 \geq r_1^*$.
  \end{itemize}	
\end{proposition}
The conclusions of Proposition~\ref{prop:contracts} are summarised in
the scatter plot in~Fig.~\ref{fig:betascatter}. Note that the
non-dominant CP always contributes a smaller fraction of its revenue
in the neutral regime. With the dominant CP, the contribution factor
is larger in the neutral regime when the revenue rates are highly
asymmetric (see the green region in Figure~\ref{fig:betascatter}, and
larger in the non-neutral regime when the revenue rates are symmetric
(see the red region in Figure~\ref{fig:betascatter}). A sufficient
condition for the former is $r_1\geq r_1^*(r_2).$ The latter
observation is of course consistent with Theorem \ref{thm:ComparisonSymmetric}, which dealt
with the case of perfect symmetry.

Proposition~\ref{prop:contracts} also establishes monotonicity
properties of the sharing contracts of $\mbox{CP}_1$  in the neutral regime in $r_1$ for a fixed $r_2.$ While
$\beta_2^{N}$ descreasess in $r_1,$ $\beta_1^{N}$
eventually decreasing in $r_1;$ see Figs.~\ref{fig:beta1a}
and~\ref{fig:beta1e}. Note that $\beta_1^{N}$ can actually be
increasing with respect to $r_1$ when the revenue rates are nearly
symmetric, in contrast with the non-neutral setting.

% shows behavior of $\beta_i, i=1,2$ in the non-neutral and neutral
% regime. When $r_1 \geq >r_2$, the non-dominant CP shares a higher
% fraction of its revenue in the non-neutral regime. This region is
% colored red and green. However the same is true for the dominant CP
% only in the region colored red. The dominant CP share a higher
% fraction of its revenue in neutral regime in the region colored green.

% While both $\beta_1^{NN}$ and $\beta_2^{NN}$ are non-increasing as
% seen from Thm.~\ref{thm:AsymBetaNN}, only $\beta_2^{N}$ is non-increasing
% in $r_1$. $\beta_1^{N}$ is non-increasing only in the region $r_1\geq
% r_1^*$ and it may be increasing or decreasing in $r_1$ satisfying
% $r_1<r_1^*$ as shown in Figs. (\ref{fig:beta1a}) and
% (\ref{fig:beta1e}). Due to this behavior of $\beta_1^{N}$, it is not
% always the case that the dominant CP contributes a higher revenue
% share to the ISP in the neutral regime for $r_1 < r_1^*;$ however,
% this is always the case for $r_1 \geq r_1^*$ as shown in
% Prop.~\ref{prop:contracts}.

% In the black colored region where $r_i/c < 1, i=1,2$ none of the CPs
% share anything in both the regimes, i.e., $\beta_i^N=\beta_i^{NN}=0$
% for all $i=1,2$. The yellow colored region $1<r_i/c <2, i=1,2$, where
% CPs revenue share is positive in the non-neutral regime and it is zero
% in the neutral regime. %Hence $\beta_i^{N}>\beta_i^{NN}$ for $i=1,2$.

\subsubsection{\textbf{Utility of CPs}}
The following proposition characterizes preference of the CPs
for the neutral and non-neutral regime.
%\begin{figure}[h!] \label{fig:CPutility}
%	\centering
%	{\includegraphics[scale=0.3]{figures/CP1utility}%
%	}
%	{\includegraphics[scale=0.3]{figures/CP2utility}%
%	}
%	\caption {Comparison of CP's utility between Non-neutral and neutral when CPs are asymmetric. We fix $c=1, r_2=2$ and vary $r_1$ from 2 to 30.}
%	\label{fig:comparison}
%\end{figure}
%
%\begin{figure}[h] \label{fig:CPUscatter}
%	\centering
%	\includegraphics[scale=0.3]{figures/CPutilityscatter}
%	\caption{Scatter plot for comparison of utility of $CP_i; i=1,2$ between non-neutral and neutral regime over different range of $r_i/c$}
%\end{figure}

\begin{proposition}
	\label{prop:CPUtility}
	Fix an $r_2$. We have
	\begin{itemize}
		\item For all $r_1>r_2$,  $\mbox{CP}_1$ prefers the non-neutral regime.
		\item For all $r_1\geq r_1^*$,  $\mbox{CP}_2$ prefers the neutral regime.
	\end{itemize}
\end{proposition}
Figure~\ref{fig:CPutilityscatter} shows the scatter plot utilities of
the players in both the regimes. Note that the dominant CP has higher
utility in the non-neutral regime as can be observed from the red and
magenta regions. This is because in the neutral regime, the dominant
CP is `forced' to pay for capacity investments that also benefit the
non-dominant~CP. Indeed, note that in the region $r_1\geq r_1^*$, the
dominant CP shares a smaller fraction of its revenue in the
non-neutral regime, but still ends-up with a higher
utility. Interestingly, the non-dominant CP obtains a higher utility
in the neutral regime when the asymmetric revenue rates are too separated (see the
pink region in Fig.~\ref{fig:CPutilityscatter}) A sufficient condition
for this is $r_1\geq r_1^*.$ This is of course due to the
`subsidization' it receives from the dominant CP. On the other hand,
when the revenue rates are nearly symmetric, even the non-dominant CP
prefers the non-neutral regime, once again consistent with
Theorem~\ref{thm:ComparisonSymmetric}. The above observations further illustrated in
Figs.~\ref{fig:CP1utility} and~\ref{fig:CP2utility}.

%However for the region $r_1< r_2^*$ the non-dominant CP
%may or may not prefer the neutral regime depending on the value of
%$r_2$ as shown in Figs.~(\ref{fig:CP1utility}) and
%(\ref{fig:CP2utility}).

% as the asymmetry between CPs increases,the CP with higher revenue per click rate (CP$_1$) continue higher utility in the non-neutral regime, however, CP with lower revenue per click rate (CP$_2$) becomes better off in the neutral regime after certain small value of $r_1$ for every fixed $r_2$. 


\subsubsection{\textbf{ISP utility}}
We next compare utility of the ISP in the non-neutral and neutral
regime. For simplicity, we take ISP utility to be the expected revenue
given as $\UISP=\mathbb{E}[\sum_{i} s(X_i)-ca_i]$ (ignoring the
risk-sensitive utility defined before). Its value in the non-neutral
regime is given by:
\[\UISP^{NN}=(1-2\beta_1^{NN})r_1+(1-2\beta_2^{NN})r_2+2c,\]
and in the neutral regime for all $r_1\geq r_1^*$ is given by:
\[\UISP^{N}=(1-2\beta_1^{N})r_1+2c.\] 
The utility for  $r_1< r_1^*$ in the neutral regime is cumbersome and we skip its expression. The following lemma demonstrates the ISPs earnings are higher in the non-neutral regime when monetization power of the dominant CP is much larger than the other, i.e., $r_1$ is much larger than $r_2$.
\begin{lemma} \label{lma:ISPutilitycomp}
	There exist $r_1^b>r_1^*$, such that for all $r_1>r_1^b$ the ISP's utility is higher in the
	 non-neutral regime.
\end{lemma}
A general comparison of ISP utility in the two regimes is not analytically
tractable. We give a numerical illustration in Figure  \ref{fig:ISPUtility}. As seen in the first figure, utility of ISP in the non-neutral
regime is higher than in the neutral regime for all $r_1$ for a  given $r_2$ and $c$.  
Scatter plot in the second figure shows that this observation extends over the entire parameter range.
\begin{figure}[h!]
	\centering
	{\includegraphics[scale=0.29]{figures/ISPutility}%
	}
	{\includegraphics[scale=0.29]{figures/ISPutilityscatter}%
	}
	\caption {The first figure compares ISP utility in neutral and non-neutral with $c=1 r_2=2$. The second figure gives a scatter plot. }
	\label{fig:ISPUtility}
\end{figure}
\subsubsection{\textbf{Social Utility}}
The social utility in the non-neutral and neutral regimes are given, respectively, as follows:
\begin{align*}
&SU^{NN}=U_{CP_1}^{NN}+U_{CP_1}^{NN}+U_{ISP}^{NN}\\
=&r_1\log\left(\frac{\beta_1^{NN}r_1}{c}\right)+r_2\log\left(\frac{\beta_2^{NN}r_2}{c}\right)-(\beta_1^{NN}r_1+\beta_2^{NN}r_2)+2c
\end{align*}
and
\begin{align*}
&SU^N=U_{CP_1}^N+U_{CP_1}^N+U_{ISP}^N\\
&=(r_1+r_2)\log\left(\frac{\beta_1^Nr_1+\beta_2^Nr_2}{c}\right)-(\beta_1^Nr_1+\beta_2^Nr_2)+2c.
\end{align*} 
\begin{figure}[h!] 
	\centering
	{\includegraphics[scale=0.29]{figures/SU}%
	}
	{\includegraphics[scale=0.29]{figures/SUscatter}%
	}
	\caption {Comparison of social utility between neutral and non-neutral regime for $c=1, r_2=2$ and scatter plot. }
	\label{fig:SocialUtility}
\end{figure}
As it is not easy to compare the social utilities analytically, we resort to numerical comparison of the utilities in Figure  \ref{fig:SocialUtility}. As seen social utility in the non-neutral regime dominates that in the neutral regime for all values of $r_1$ for a given $r_2$ and $c$. The scatter plot in the second part of the figure shows that the observation continue to hold for all parameters.
\subsubsection{\textbf{Total Effort by ISP}}
Finally we compare the total effort by ISP for CPs in the non-neutral and neutral regime given, respectively, as follows
\begin{align*}
A^{NN}&=a_1^{NN}+a_2^{NN}=\frac{\beta_1^{NN}r_1}{c}-1+\frac{\beta_2^{NN}r_2}{c}-1\\
&=\frac{\frac{r_1}{c}}{W(\frac{r_1}{c}e)}+\frac{\frac{r_2}{c}}{W(\frac{r_2}{c}e)}-2 \;\; \forall \; r_1>r_1^*,
\end{align*}
and
\begin{align*}
A^{N}=2a^{N}=2\left(\frac{\beta_1^{N}r_1}{2c}-1\right)=\frac{\frac{r_1}{c}}{W(\frac{r_1}{2c}e)}-2 \hspace{.75mm}\forall \hspace{.75mm}r_1>r_1^*
\end{align*}
\begin{figure}[!t] \label{fig:TotalEffort}
	\centering
	{\includegraphics[scale=0.29]{figures/totaleffort}%
	}
	{\includegraphics[scale=0.35]{figures/totaleffortscatter}%
	}
	\caption{Scatter plot for comparison between total effort (investment) by ISP in non-neutral and neutral regime over different range of $r_i/c$}
\end{figure}
\begin{lemma} \label{lma:totaleffortcomp}
	There exist a threshold $r_1^a>r_1^*$ such that total effort by ISP is higher in neutral regime than in the  non-neutral. The threshold satisfies the following:
\end{lemma}
The threshold $r_1^a$ is given by following equation:
$$r_1^a \left(\frac{1}{W(\frac{r_1^a}{2c}e)}-\frac{1}{W(\frac{r_1^a}{c}e)}\right)=\frac{{r_2}}{W(\frac{r_2}{c}e)}$$
It can be seen from above equation that $r_1^a$ is monotonically increasing in $r_2$.\\

The above lemma implies that total effort by ISP in the neutral regime becomes higher when there is high asymmetry between CP's revenue per click rates. 

==> Journal Version Arxiv/GeneralCase.tex <==
%\section{Comparison between neutral and non-neutral regime}In numerical comparisons we fix $r_2$ and
$c$ and vary $r_1$.
\subsubsection{\textbf{Contracts}}
The following proposition provides a comparison of the equilibrium
contracts in both the regimes.

\begin{figure*}[!t]
	\centering
	\subfloat[]{\includegraphics[scale=0.05]{figures/betascatter}\label{fig:betascatter}}
			\hspace{0.4cm}
	\subfloat[]{\includegraphics[scale=0.3]{figures/beta1a}
		\label{fig:beta1a}}
	\hspace{0.4cm}
	\subfloat[]{\includegraphics[scale=0.3]{figures/beta1e}
		\label{fig:beta1e}}
	\vspace{-.3cm}
	\caption {(\ref{fig:betascatter}) gives scatter-plot of $\beta$s. (\ref{fig:beta1a}) and (\ref{fig:beta1e}) gives variation of equilibrium $\beta_1$ vs $r_1$ under neutral and non-neutral regime.}
	\label{fig:beta}
\end{figure*}

\begin{figure*}[!h]
	\centering
	
	\subfloat[]{\includegraphics[scale=0.3]{figures/CPutilityscatter}		\label{fig:CPutilityscatter}}
	\hspace{0.4cm}
	\subfloat[]{\includegraphics[scale=0.3]{figures/CP1utility}\label{fig:CP1utility}}
	\hspace{0.4cm}
	\subfloat[]{\includegraphics[scale=0.3]{figures/CP2utility}\label{fig:CP2utility}}
	\vspace{-.3cm}
	\caption {(\ref{fig:CPutilityscatter}) shows scatterplot for the CP utilities at equilibrium. (\ref{fig:CP1utility})\&(\ref{fig:CP2utility}) compare $\mbox{CP}_1$ utility in both regimes as $r_1$ varies.}
	\label{fig:CPUtility}
\end{figure*}


 
 \begin{proposition} 
 	\label{prop:contracts}
 	Fix $r_2 > 0.$ We have
 	\begin{itemize}
 		\item For $r_1\geq r_2$, $\beta_2^{NN} \geq \beta_2^{N}$.  $\beta_2^{N}$ decreases in $r_1$.
 		\item  For $r_1\geq r_1^*$, $\beta_1^{N}>\beta_1^{NN}$.  $\beta_1^{N}$ decreases in $r_1$ for $r_1>r_1^*$. 
 	\end{itemize}	
 \end{proposition}
 
Fig. (\ref{fig:betascatter}) shows behavior of $\beta_i, i=1,2$ in the
non-neutral and neutral regime. When $r_1 \geq >r_2$, the non-dominant
CP shares a higher fraction of its revenue in the non-neutral
regime. This region is colored red and green. However the same is true
for the dominant CP only in the region colored red. The dominant CP
share a higher fraction of its revenue in neutral regime in the region
colored green.

While both $\beta_1^{NN}$ and $\beta_2^{NN}$ are non-increasing as
seen from Thm.~\ref{Thm:NN-asy}, only $\beta_2^{N}$ is non-increasing
in $r_1$. $\beta_1^{N}$ is non-increasing only in the region $r_1\geq
r_1^*$ and it may be increasing or decreasing in $r_1$ satisfying
$r_1<r_1^*$ as shown in Figs. (\ref{fig:beta1a}) and
(\ref{fig:beta1e}). Due to this behavior of $\beta_1^{N}$, it is not
always the case that the dominant CP contributes a higher revenue
share to the ISP in the neutral regime for $r_1 < r_1^*;$ however,
this is always the case for $r_1 \geq r_1^*$ as shown in
Prop.~\ref{prop:contracts}.

In the black colored region where $r_i/c < 1, i=1,2$ none of the CPs
share anything in both the regimes, i.e., $\beta_i^N=\beta_i^{NN}=0$
for all $i=1,2$. The yellow colored region $1<r_i/c <2, i=1,2$, where
CPs revenue share is positive in the non-neutral regime and it is zero
in the neutral regime. %Hence $\beta_i^{N}>\beta_i^{NN}$ for $i=1,2$.

\subsubsection{\textbf{Utility of CPs}}
In this subsection we compare the utilities of the CPs in both the
regimes. The following proposition characterizes preference of the CPs
for the neutral and non-neutral regime.
%\begin{figure}[h!] \label{fig:CPutility}
%	\centering
%	{\includegraphics[scale=0.3]{figures/CP1utility}%
%	}
%	{\includegraphics[scale=0.3]{figures/CP2utility}%
%	}
%	\caption {Comparison of CP's utility between Non-neutral and neutral when CPs are asymmetric. We fix $c=1, r_2=2$ and vary $r_1$ from 2 to 30.}
%	\label{fig:comparison}
%\end{figure}
%
%\begin{figure}[h] \label{fig:CPUscatter}
%	\centering
%	\includegraphics[scale=0.3]{figures/CPutilityscatter}
%	\caption{Scatter plot for comparison of utility of $CP_i; i=1,2$ between non-neutral and neutral regime over different range of $r_i/c$}
%\end{figure}



\begin{proposition}
\label{prop:CPUtility}
Fix an $r_2$. We have
\begin{itemize}
	\item For all $r_1>r_2$, the dominant CP prefers the non-neutral regime.
	\item For all $r_1\geq r_1^*$,  the non dominant CP prefers the neutral regime.
\end{itemize}
\end{proposition}

Figure \ref{fig:CPUtility} shows the scatter plot utilities of the
players in both the regimes. For $r_1\geq >r_2$, the dominant CP has
higher utility in the non-neutral regime as can be observed from the
red and magenta regions. This is because in the neutral regime, the
dominant CP is `forced' to pay for capacity investment that benefits
the non-dominant CP. Indeed, note that in the region $r_1\geq r_1^*$,
the dominant CP shares a smaller fraction of its revenue in the
non-neutral regime, but still ends-up with a higher utility. In this
region, the non-dominant CP obtains higher utility in the neutral
regime (thanks to the `subsidization' from the dominant CP) and hence
prefers it. However for the region $r_1< r_2^*$ the non-dominant CP may or may not prefer the neutral regime depending on the value
of $r_2$ as shown in Figs.~(\ref{fig:CP1utility}) and
(\ref{fig:CP2utility}).
% as the asymmetry between CPs increases,the CP with higher revenue per click rate (CP$_1$) continue higher utility in the non-neutral regime, however, CP with lower revenue per click rate (CP$_2$) becomes better off in the neutral regime after certain small value of $r_1$ for every fixed $r_2$. 


\subsubsection{\textbf{Utility of ISP}}
We next compare utility of the ISP in the non-neutral and neutral
regime. For simplicity, we take ISP utility to be the expected revenue
given as $\UISP=\mathbb{E}[\sum_{i} s(X_i)-ca_i]$ (ignoring the
risk-sensitive utility defined before). Its value in the non-neutral
regime is given by:
\[\UISP^{NN}=(1-2\beta_1^{NN})r_1+(1-2\beta_2^{NN})r_2+2c,\]
and in the neutral regime for all $r_1\geq r_1^*$ is given by:
\[\UISP^{N}=(1-2\beta_1^{N})r_1+2c.\] 
The utility for  $r_1< r_1^*$ in the neutral regime is cumbersome and we skip its expression. The following lemma demonstrates the ISPs earnings are higher in the non-neutral regime for monetization power of the dominant CP is much larger than the other, i.e., $r_1$ is much larger than $r_2$.
\begin{lemma} \label{lma:ISPutilitycomp}
	There exist $r_1^b>r_1^*$, such that for all $r_1>r_1^b$ ISP
        has better utility in the non-neutral regime.
\end{lemma}

Comparison of the ISP utilities in general is not analytically
tractable. We thus plot it under neutral and non-neutral regime in
Fig.~ \ref{fig:ISPUtility}. As seen in the first figure, ISP for a
fixed $r_2$ and $c$, for all $r_1$ utility of ISP in the non-neutral
regime is higher than in the. Also, we can observe the same behavior
is the scatter plot given in the second figure.
%neutral one. That is for all $r_1\geq r_2$ ISP is better off  in non-neutral regime than in neutral. Same analysis is true for the case where $r_2>r_1$, and thus, ISP is always better off in non-neutral regime. Figure \ref{fig:ISPscatterplot} also shows that ISP is always better off in non-neutral regime.


\begin{figure}[h!]
	\centering
	{\includegraphics[scale=0.29]{figures/ISPutility}%
	}
	{\includegraphics[scale=0.29]{figures/ISPutilityscatter}%
	}
	\caption {Comparison of ISP utility between Non-neutral $c=1, r_2=2$ and scatter plot. }
	\label{fig:ISPUtility}
\end{figure}

\subsubsection{\textbf{Social Utility}}
Finally, we compare social utility in both the regimes. In the non-neutral regime, social utility is given by
\begin{align*}
SU^{NN}=&U_{CP_1}^{NN}+U_{CP_1}^{NN}+U_{ISP}^{NN}\\
=&r_1\log\left(\frac{\beta_1^{NN}r_1}{c}\right)+r_2\log\left(\frac{\beta_2^{NN}r_2}{c}\right)-(\beta_1^{NN}r_1+\beta_2^{NN}r_2)+2c.
\end{align*} 
Similarly, social utility in the neutral case is given as
\begin{align*}
&SU^N=U_{CP_1}^N+U_{CP_1}^N+U_{ISP}^N\\
&=(r_1+r_2)\log\left(\frac{\beta_1^Nr_1+\beta_2^Nr_2}{c}\right)-(\beta_1^Nr_1+\beta_2^Nr_2)+2c.
\end{align*} 
\begin{figure}[h!] \label{fig:SocialUtility}
	\centering
	{\includegraphics[scale=0.29]{figures/SU}%
	}
	{\includegraphics[scale=0.29]{figures/SUscatter}%
	}
	\caption {Comparison of social utility between neutral and non-neutral regime for $c=1, r_2=2$ and scatter plot. }
\end{figure}
As it is not easy to compare the social utilities analytically, we do numerical comparison in the first part of Fig.5. As seen social utility in the non-neutral regime dominates that in the neutral regime for all values of $r_1$ for a given $r_2$ and $c$. The scatter plot in the second part of the figure also gives the same observation.
\subsubsection{\textbf{Total Effort by ISP}}
In this section, we compare the total effort by ISP for CPs in the non-neutral and neutral regime. We focus on the region where $r_1>r_1^*$. Total effort in non-neutral for all $r_1$ regime is given by
\begin{align*}
	A^{NN}&=a_1^{NN}+a_2^{NN}=\frac{\beta_1^{NN}r_1}{c}-1+\frac{\beta_2^{NN}r_2}{c}-1\\
	&=\frac{\frac{r_1}{c}}{W(\frac{r_1}{c}e)}+\frac{\frac{r_2}{c}}{W(\frac{r_2}{c}e)}-2
\end{align*}
Similarly, total effort in neutral regime is
\begin{align*}
	A^{N}=2a^{N}=2\left(\frac{\beta_1^{N}r_1}{2c}-1\right)=\frac{\frac{r_1}{c}}{W(\frac{r_1}{2c}e)}-2 \hspace{.75mm}\forall \hspace{.75mm}r_1>r_1^*
\end{align*}
\begin{figure}[!t] \label{fig:TotalEffort}
	\centering
	{\includegraphics[scale=0.29]{figures/totaleffort}%
	}
	{\includegraphics[scale=0.35]{figures/totaleffortscatter}%
	}
	\caption{Scatter plot for comparison between total effort (investment) by ISP in non-neutral and neutral regime over different range of $r_i/c$}
\end{figure}
\begin{lemma} \label{lma:totaleffortcomp}
	There exist some $r_1^a$ sufficiently larger than $r_1^*$, s.t. for all $r_1^a>r_1^*$, total effort by ISP is higher in neutral regime than in the  non-neutral.
\end{lemma}
The threshold $r_1^a$ is given by following equation:
$$r_1^a \left(\frac{1}{W(\frac{r_1^a}{2c}e)}-\frac{1}{W(\frac{r_1^a}{c}e)}\right)=\frac{{r_2}}{W(\frac{r_2}{c}e)}$$
It can be seen from above equation that $r_1^a$ is monotonically increasing in $r_2$.\\

The above lemma implies that total effort by ISP in the neutral regime becomes higher when there is high asymmetry between CP's revenue per click rates. 

==> Journal Version Arxiv/MultiSymmetry.tex <==
In this section we consider the symmetric case where revenue per unit
demand for all the CPs is the same, i.e., $r_1=r_2, \ldots,=r_n := r.$
In other words, the CPs are symmetric with regards to the ability to
monetize their content.
% Let $r$ denote this common value.
In this setting, we analyze the equilibrium contracts arising in the
neutral as well as non-neutral regime, and the resulting surplus of
the CPs and the ISP. Our results highlight, surprisingly, that even
when the CPs are symmetric, the imposition of neutrality actually
shrinks the surplus of all parties involved. Moreover, this `loss of
surplus' becomes more pronounced as the number of CPs $n$ grows.

%We begin with the non-neutral regime. 

\subsection{Non-neutral regime}
% Under the neutral regime and linear contracts, the IC constraint of
% the ISP, i.e.,
% $\max_{a_i}E_{X_1,\;X_2}[H(s_1(X_1),s_2(X_2),a_i,a)]$, simplifies to
% $\max_a \sum_i(\beta_ir_i\log(a_i+1)-ca_i)$.  The optimal effort
% level for the non-neutral regime in this case for a given contract
% $\beta_i, i=1,2,...n$ for each $\CPi$ is given by:
%\begin{equation}
%a^*_i=\max\left(\frac{\beta_i r}{c}-1,0\right).
%\end{equation}
In the non-neutral regime, it is easy to see that when
$\overline{H}=-1$, the interactions between each CP and the ISP are
decoupled. The optimization problem in (\ref{eqn:OptNonNeutral}) for
$CP_i, i\in N,$ after substituting the optimal effort simplifies to:
\begin{align*}
	&\max_{\beta_i\in [0,1]} \hspace{2mm} (1-\beta_i)r\log\left(\max\left(\frac{\beta_ir}{c},1\right)\right).
\end{align*}
Moreover, we note that it is only interesting to consider the case
$r > c.$ Indeed, since the monetization resulting from ISP effort
$a_i$ for CP~$i$ equals $r\log(1+a_i),$ the marginal monetization is
at most $r.$ Thus, if $r \leq c,$ it is not worthwhile for CPs to make
any investments to grow the demand.


%Let  $W(\cdot)$ denote the stand LambertW function \textcolor{blue}{\cite{}} taking values on the principle branch. The optimal contract is characterized in term LambertW function in the following. %Each CP has his own constraint optimization problem with common constraint which is the optimization problem of the ISP. Then, the global problem can be seen as a hierarchical non-cooperative game between CPs (here 2 leaders) and one ISP (one follower).Usually, this type of complex game involves the framework of Generalized Nash Equilibrium Point (GNEP) and tools from it mainly for optimization theory and KKT conditions. In our setting, we are able to determine explicitly the equilibrium solution of this hierarchical game between two CPs and one ISP.

The following result characterizes the equilibrium contracts between
each CP and the ISP. The contracts are expressed in terms of the
LambertW function computed on its principle branch, denoted as
$W(\cdot)$ (see~\cite{corless1996lambertw}).
% The following theorem gives equilibrium contracts, efforts and
% utilities in the non-neutral regime in terms of the LambertW
% function.
\begin{thm}
  \label{thm:equillibrium-NN}
  If $r > c,$ the equilibrium contract between $\CPi, i \in \mathcal{N}$ and the
  ISP is given by 
  \begin{equation} \label{eqn:SymmetricBetaNN}
    \beta^{NN}:=\beta^{NN}_i= \frac{1}{W\left(\frac{r}{c}e\right)}.    
  \end{equation}
\end{thm}
Since $W(\cdot)$ in strictly increasing and $W(e) = 1,$ it follows
that $\beta^{NN} \in (0,1)$ when $r/c > 1.$ Moreover, note that
equilibrium fraction $\beta^{NN}$ of CP revenue that is shared with the
ISP is a strictly decreasing function of the ratio $r/c,$ as might be
expected.

Using Theorem~\ref{thm:equillibrium-NN}, one can easily characterize
the equilibrium effort of the ISP as well as the surplus of each
agent.
\begin{cor}
  \label{cor:equillibrium-NN}
  Assume $r > c.$ The equilibrium effort for each $\CPi, i \in \mathcal{N}$ put
  by the ISP is given by
  \begin{equation} \label{eqn:SymmetricEffortNN}
    a^{NN}:=a^{NN}_i= \frac{r\beta^{NN} }{c}-1 > 0.
  \end{equation}
  The equilibrium surplus of $\CPi, i \in \mathcal{N}$ is given by
  \begin{equation}
    \label{eqn:SymmetricCPUtilityNN}
    \UCPi^{NN}=(1-\beta^{NN}) r\log(a^{NN}+1)
    =\frac{(1-\beta^{NN})^2}{\beta^{NN}}r > 0.
  \end{equation}
  Finally, the equilibrium surplus of the ISP is given by
  \begin{equation}
    \label{eqn:SymmetricISPUtilityNN}
    \UISP^{NN}=nr+nc-2n\beta^{NN}r > 0.
  \end{equation}
\end{cor}

Note that so long as $r>c,$ the equilibrium contracts award each CP
and the ISP a positive surplus.

%As the optimization problem decouples in the non-neutral regime, the
%equilibrium contracts, efforts and CP utility are independent of
%$n$. Each CP shares a positive fraction of their revenue with the ISP
%only if $r/c>1$, otherwise none of the CPs will share their revenue
%with the ISP. Further, this share at equilibrium is decreasing in $r$
%while increasing in $c$ {\bf (better to give some intuition here)}.

\subsection{Neutral regime}

We now consider the neutral regime. The CPs are still assumed to be
symmetric, only the ISP is now \emph{constrained} to make the same
investment decision for all CPs, i.e., $a_1=\ldots=a_n:=a $.  The
surplus of $\CPi$ in this case, after substituting the
optimal ISP effort simplifies to:
\begin{align*}
  (1-\beta_i)r\log\left(\max\left(\frac{\sum_{j=1}^{n}\beta_jr}{nc},1\right)\right).
\end{align*} 
Since the surplus of each CP in the neutral regime depends on the
actions of all CPs, we seek contract profiles $(\beta^N_i, i \in N)$ that
constitute a \emph{Nash equilibrium} between CPs. These equilibria are
characterized completely in the following theorem. As before, the only
scenario of interest is $r >c.$

\begin{thm}
  \label{thm:equillibrium-N}
  Consider the neutral regime with $r > c.$ In this case, only
  symmetric Nash equilibria exist. When $1 < r/c \leq n,$ there are
  two Nash equilibria, $\boldsymbol{0},$ and $(\beta^N_i, i \in \mathcal{N}),$
  where
  \begin{equation}
    \label{eqn:SymmetricBetaN}
    \beta_i^N = \beta^N := \frac{1}{nW\left(\frac{r}{nc}e^{1/n}\right)}.
  \end{equation}
  When $r/c > n,$ $(\beta^N_i, i \in \mathcal{N})$ is the only Nash equilibrium,
  where $\beta_i^N$ is given by \eqref{eqn:SymmetricBetaN}.
\end{thm}

Note that when $1 < r/c \leq n,$ unlike in the non-neutral regime,
making no contributions to the ISP, resulting in zero suplus for all
parties, is an equilibrium between the CPs. The other equilibrium,
given by \eqref{eqn:SymmetricBetaN}, results in a positive surplus for
all parties (as is shown in the following corollary). In the remainder
of this section, we will refer to this latter equilibrium as the
\emph{non-zero} equilibrium.

\begin{cor}
  Consider the neutral regime, with $r > c.$ Under the non-zero
  equilibrium:
  \begin{itemize}
  \item The effort for $\CPi, i \in N$, put by the ISP is given by
    \begin{equation} \label{eqn:SymmetricEffortN}
      a^N:=a_i^N(n)=\max\left(\frac{\beta^N r}{c}-1,0\right).
    \end{equation}
  \item The surplus of $\CPi, i\in N$ is given by
    \begin{equation}
      \label{eqn:SymmetricCPUtility}
      \UCPi^{N}=(1-\beta^{N}) r\log(a^{N}+1)
      =\frac{\left(1-\beta^{N}\right)^2}{n\beta^{N}}r > 0.
    \end{equation}
  \item The surplus of ISP is given by
    \begin{equation}
      \label{eqn:SymmetricISPUtility}
      \UISP^{N}=r+nc-(n+1)\beta^{N}r > 0.
    \end{equation}
  \end{itemize}
\end{cor}

% Each CP shares a positive fraction of their revenue in the neutral
% regime if $r/c >n$ and nothing is shared if $r/c \leq 1$. In the
% region $1<r/c\leq n$, two equilibrium are possible, in which either
% nothing is shared or a strictly positive fraction of the revenue is
% shared. Further, like in the case of non-neutral regime, the revenue
% shared at equilibrium is a decreasing function of $r$ and an
% increasing function of $c$.

\subsection{Neutral regime v/s Non-neutral regime}

Having now characterized the equilibrium contracts and the surplus of
each CP and the ISP under the neutral and the non-neutral regime, we
are now in a position to compare the two. As the following result
shows, the non-neutral regime is actually better \emph{for all
  parties} as compared to the neutral regime.
\begin{thm}
  \label{thm:ComparisonSymmetric}
  Suppose $r > c,$ and $n \geq 2.$ In the symmetric case, at
  equilibrium, the following statements hold.
  \begin{enumerate}
  \item CPs share a higher fraction of their revenue with the ISP in
    the non-neutral regime, i.e., $\beta^{NN} > {\beta^{N}}.$
  \item The effort by the ISP for each CP is higher in the non-neutral
    regime, i.e., $a^{NN} > {a^{N}}$
  \item The surplus of each CP is higher in the non-neutral regime,
    i.e., $\UCPi^{NN}> \UCPi^N$ for all $i \in N$
  \item The surplus of the ISP is higher in the non-neutral regime,
    i.e., $\UISP^{NN} > \UISP^N$.
  \end{enumerate}
\end{thm}
The above result highlights that, surprisingly, constraining the ISP
to be neutral is actually sub-optimal for all parties, even when the
CPs are symmetric. In other words, the non-neutral regime is actually
preferable to the ISP as well as the CPs. Intuitively, the reason for
this \emph{tragedy of the commons} is that the imposition of
neutrality skews the payoff landscape for each CP, such that the
`benefit' of any additional investment it makes gets `shared' across
all CPs. This induces the CPs to commit smaller fractions of their
revenues to the ISP, which in turn results in a lower ISP effort, and
a lower demand growth for all CPs. Indeed, as we show below, this
effect gets further magnified with an increase in the number of CPs.

% The above result indicated that each CP gives a higher share of
% their revenue to the ISP in the non-neutral regime than in the
% neutral regime and in turn the ISP puts more efforts in the
% non-neutral for each CP than in the neutral regime. Further, the
% utilities of both CPs and the ISP is higher in the non-neutral
% regime than in the neutral regime, i.e., the non-neutral regime is
% preferred by both the CPs and the ISP. The fact that the ISP is
% forced to put equal efforts for all CPs deincentivizes them from
% sharing higher amount as any CP sharing lower amount will also get
% equal effort from the ISP as they do. Reduced share will make ISP
% put lesser effort which in turns reduces the demand for CPs content
% lowering their net utility. Due to the reduced share from the CPs,
% ISP utility also reduces.
%
%\begin{lemma} \label{lma:betacomparision:gen}
%	Proportion of revenue shared by each CP in higher in non-neutral regime as compared to that in neutral regime, i.e.,	$\beta^{NN} \geq {\beta^{N}}$
%\end{lemma}
%Above lemma suggest that CPs share more revenue in non-neutral regime as compared to neutral regime.
%
%\begin{lemma} \label{lma:effort:gen}
%	ISP makes more investment in the non-neutral regime than in the neutral regime, i.e.,	
%\end{lemma} 
%
%
%
%\begin{lemma} \label{lma:UISPcomp:gen}
%	Utility of ISP is higher in non-neutral regime as compared to that in neutral regime.
%\end{lemma}
%
%\begin{lemma} \label{lma:UCPcomp:gen}
%	Utility of each CP is higher in non-neutral regime as compared to that in neutral regime.
% \end{lemma}

\subsection{The effect of number of CPs}

In the non-neutral regime, the interactions between the different CPs
and the ISP are decoupled, implying that the impact of scaling $n$ is
trivial. Thus, we now study the impact of scaling $n$ in the
neutral regime, on the equilibrium ISP effort, and the surplus of each
agent. Note that when $n=1,$ the neutral and the non-neutral regime
coincide. Our main result is the following.

% However, for $n>1$ the behavior in the neutral regime can change as
% the effort decisions of ISP are coupled across the CPs, whereas it
% remains the same in the non-neutral regime (as in the case $n=1$)
% due to the decoupled nature of contract between the CPs and the
% ISP. Thus the results for the neutral regime with $n=1$ explains the
% behavior of the non-entral regime and it is enoguh to focus on the
% behavior in the neutral regime as $n$ varies. The following theorem
% summarizes the observations in the neutral regime.

\begin{thm}
  \label{thm:EffectOfCPsize}
  Suppose that $r > c.$ In the neutral regime, the non-zero
  equilibrium satisfies the following properties.
\begin{enumerate}
\item $\beta^N$ is a strictly decreasing function of $n.$
\item The effort by the ISP for each CP ($a^N$) is a strictly
  decreasing function of $n,$ even though the total effort ($na^N$) by
  the ISP is a strictly increasing function of $n.$  
\item The surplus of each CP is a strictly decreasing function of $n,$
  and $\lim_{n \rightarrow \infty} U^N_{CP_i}(n) = 0.$
\item The surplus of the ISP is eventually strictly decreasing in $n,$
  and $\lim_{n \rightarrow \infty} U^N_{ISP}(n) = 0.$
  % receives from each CP decreases. His a strictly decreasing
  % function of $n.$owever, the total utility first increases for all
  % $n$ satisfying
  % $n^2+n+1<n W\left(\frac{r}{nc}e^\frac{1}{n}\right)$. For lareger
  % $n$ the ISP utility deceases and approaches zero as
  % $n\rightarrow \infty$.
\end{enumerate} 
\end{thm}

Theorem~\ref{thm:EffectOfCPsize} highlights that an increase in the
number of CPs further exacerbates the sub-optimality of the neutral
regime for the CPs as well as the ISP. As before, the explanation for
this is that with increasing $n,$ the surplus resulting from an
additional contribution by any $CP$ gets `split' further, thus
disincentivising the CPs from offering a significant fraction of their
revenues to the ISP. The variation of ISP utility as a function of $n$ is depicted in Figure \ref{fig:neutral_n_variation_ISP} for different values of $r/c$. In all cases, the utility first increase for some $n$ and the decreases thereafter.  

%The conclusions of
%Theorem~\ref{thm:EffectOfCPsize} are illustrated in
%Figure~\ref{fig:neutral_n_variation}. The eventual monotonicity of ISP
%surplus with $n$ is illustrated in
%Figure~\ref{fig:neutral_n_variation_ISP}. \jk{I seem to have altered
%  the way the first figure renders. To be fixed.}


%\begin{lemma} \label{lma:beta-N}
%	$\beta^N$ decreases with increase in n.
%\end{lemma}
%
%\begin{lemma} \label{lma:effort-N}
%	Individual effort for each CP by ISP, $a^N$ decreases with increase in n. However, total effort increases with increase in $n$.
%\end{lemma}
%
%\begin{lemma} \label{lma:UCP-N}
%	Utility of each CP decreases with increase in n.
%\end{lemma}
%
%\begin{lemma} \label{lma:ISPU-N}
%	Fraction of ISP utility from each CP decreases with increase in n. However, total utility first increases for all $n$ satisfying $n^2+n+1<n W\left(\frac{r}{nc}e^\frac{1}{n}\right)$.\\
%%	\begin{equation}
%%	n^2+n+1<n W\left(\frac{r}{nc}e^\frac{1}{n}\right)
%%	\end{equation}
%	As $n$ becomes larger, this inequality no longer holds, then ISP utility starts deceasing and approaches to  zero as $n\rightarrow \infty$.
%\end{lemma}

%{\bf Results to be discussed:} As number of CPs increase, the
% proportion of the revenue by each CP they share with ISP decreases
% which in turn reduces the effort ISP puts for each CP. However, it
% is interesting to note that the total effort by ISP increases with
% the number of CPs.


%\begin{figure}[h!] 
%	\centering
%	{\includegraphics[scale=0.27]{figures/beta_n}%
%	}
%	{\includegraphics[scale=0.27]{figures/effort_n}%
%	}
%	{\includegraphics[scale=0.27]{figures/totaleffort_g}%
%	}
%	{\includegraphics[scale=0.27]{figures/CPU_n}%
%	}
%	{\includegraphics[scale=0.27]{figures/ISPU_n}%
%	}
%	\caption {Comparison between Non-neutral and neutral regime
%          when CPs are symmetric w.r.t. $n$. We fix $c=1, r=20.1$ and
%          vary $n$ from 1 to 20.}
%        \label{fig:neutral_n_variation}
%\end{figure}

\begin{figure}[h!] 
	\centering
%	{\includegraphics[scale=0.35]{figures/ISPUa}%
%	}
	{\includegraphics[scale=0.225]{figures/ISPUc}%
	}
	{\includegraphics[scale=0.225]{figures/ISPUd}%
	}
	{\includegraphics[scale=0.225]{figures/ISPUe}%
	}
%	{\includegraphics[scale=0.35]{figures/ISPUf}%
%	}
%	{\includegraphics[scale=0.225]{figures/ISPUg}%
%	}
	\caption {ISP utility in the neutral regime
          as $n$ varies for different $r/c$.}
        \label{fig:neutral_n_variation_ISP}
\end{figure}
%=%Again, $W(\frac{1}{n}e^\frac{1}{n})$ is a decreasing function in $n$,\\
% $\implies\frac{W(\frac{1}{n}e^\frac{1}{n})}{W(\frac{1}{(n+1)}e^\frac{1}{n+1})} \geq 1$\\
%
% \begin{align*}
% \frac{\partial f(n,1)}{\partial n}&=\frac{1}{(n+1)^2}\cdot\frac{W(\frac{1}{n}e^\frac{1}{n})}{W(\frac{1}{(n+1)}e^\frac{1}{n+1})}\\
%  +\frac{n}{n+1}\cdot&\frac{1}{W^2(\frac{1}{(n+1)}e^\frac{1}{n+1})} \bigg\{W(\frac{1}{n}e^\frac{1}{n})W'(\frac{1}{(n+1)}e^\frac{1}{n+1})-W(\frac{1}{n}e^\frac{1}{n})W'(\frac{1}{(n+1)}e^\frac{1}{n+1})\bigg\}\\
%  &=\frac{1}{(n+1)^2}\cdot\frac{W(\frac{1}{n}e^\frac{1}{n})}{W(\frac{1}{(n+1)}e^\frac{1}{n+1})}\\
%   +\frac{n}{n+1}\cdot&\frac{1}{W^2(\frac{1}{(n+1)}e^\frac{1}{n+1})} \Bigg\{ \frac{W(\frac{1}{n}e^\frac{1}{n})\left(\frac{-1}{n^2}e^\frac{1}{n}-\frac{1}{n^3}e^\frac{1}{n}\right)}{\frac{1}{n}e^\frac{1}{n}\left(1+W(\frac{1}{n}e^\frac{1}{n})\right)}\cdot W(\frac{1}{(n+1)}e^\frac{1}{n+1})\\
%   & -\frac{W(\frac{1}{(n+1)}e^\frac{1}{(n+1)})\left(\frac{-1}{(n+1)^2}e^\frac{1}{(n+1)}-\frac{1}{(n+1)^3}e^\frac{1}{(n+1)}\right)}{\frac{1}{(n+1)}e^\frac{1}{(n+1)}\left(1+W(\frac{1}{(n+1)}e^\frac{1}{(n+1)})\right)}\cdot W(\frac{1}{n}e^\frac{1}{n})\Bigg \}\\
%   &=\frac{1}{(n+1)^2}\cdot\frac{W(\frac{1}{n}e^\frac{1}{n})}{W(\frac{1}{(n+1)}e^\frac{1}{n+1})}\\
%    &+\frac{n}{n+1}\cdot \frac{W(\frac{1}{n}e^\frac{1}{n})}{W(\frac{1}{(n+1)}e^\frac{1}{n+1})} \Bigg \{ -\frac{n+1}{n^2\left(1+W(\frac{1}{n}e^\frac{1}{n})\right)}\\
%    &+\frac{n+2}{(n+1)^2\left(1+W(\frac{1}{n+1}e^\frac{1}{(n+1)})\right)} \Bigg \}\\
%    &=\frac{1}{(n+1)^2}\cdot\frac{W(\frac{1}{n}e^\frac{1}{n})}{W(\frac{1}{(n+1)}e^\frac{1}{n+1})}  \Bigg \{ 1+\\
%    &\frac{-(n+1)^3\left(1+W(\frac{1}{n+1}e^\frac{1}{(n+1)})\right)+n^2(n+2)\left(1+W(\frac{1}{n}e^\frac{1}{n})\right)}{n(n+1)\left(1+W(\frac{1}{n}e^\frac{1}{n})\right)\left(1+W(\frac{1}{n+1}e^\frac{1}{(n+1)})\right)} \Bigg \}
%   	 	\end{align*}
%Utility of each CP is given as 
%\begin{align*}
%U_{CP}^{N}&=(1-\beta^{N})r\log\left(\frac{\beta^{N}r}{c}\right)\\
%&=(1-\beta^{N})r\frac{(1-\beta^{N})}{n\beta^{N}}\\
%&=\frac{(1-\beta^{N})^2}{n\beta^{N}}r
%\end{align*}




%$$\iff 1+2W\left(\frac{a}{n}e^\frac{1}{n}\right)<n^2W^2\left(\frac{a}{n}e^\frac{1}{n}\right)+2nW^2\left(\frac{a}{n}e^\frac{1}{n}\right)$$
%\begin{equation}
%\iff \frac{(1+\frac{1}{n})^2}{(1+\frac{2}{n})}<\frac{\left(1+W\left(\frac{a}{n}e^\frac{1}{n}\right)\right)^2}{\left(1+2W\left(\frac{a}{n}e^\frac{1}{n}\right)\right)}
%\end{equation}
%$$
%\iff \frac{1+2W\left(\frac{a}{n}e^\frac{1}{n}\right)}{1+\frac{2}{n}}<\left(\frac{1+W\left(\frac{a}{n}e^\frac{1}{n}\right)}{1+\frac{1}{n}}\right)^2
%$$
%$$
%\iff \frac{n}{n+2}\cdot\left(1+2W\left(\frac{a}{n}e^\frac{1}{n}\right)\right)<\left(\frac{n}{n+1}\right)^2\cdot \left(1+W\left(\frac{a}{n}e^\frac{1}{n}\right)\right)^2
%$$
%which is true since $\frac{n}{n+2}<\left(\frac{n}{n+1}\right)^2$ and $\left(1+2W\left(\frac{a}{n}e^\frac{1}{n}\right)\right)<\left(1+W\left(\frac{a}{n}e^\frac{1}{n}\right)\right)^2$\\
%\begin{equation}
%\iff \frac{(1+\frac{1}{n})^2}{(1+\frac{2}{n})}<\frac{\left(1+W\left(\frac{a}{n}e^\frac{a}{n}\right)\right)^2}{\left(1+2W\left(\frac{a}{n}e^\frac{a}{n}\right)\right)}
%\end{equation}
%$$\iff \frac{(1+\frac{1}{n})^2}{(1+\frac{2}{n})}<\frac{\left(1+W\left(\frac{a}{n}e^\frac{a}{n}\right)\right)^2}{\left(1+2W\left(\frac{a}{n}e^\frac{a}{n}\right)\right)}$$
%Since, $n\beta^N(n)$ is increasing in $n$,LHS>0, and c/r<1. Thus last inequality holds.
%\begin{lemma}
%	Utility of each CP decreases with increase in n.
%\end{lemma}
%\textbf{Proof:}
%We know that each CP maximizes over its utility which is for any $n$ given as:
%$$U_{CP}^N(n)=(1-\beta^{N}(n))r\log\left(\frac{\beta^{N}(n)r}{c}\right)$$
%Since, the above function is concave in $\beta$ and we know that $\beta^N(n)\le \beta^N(m) \forall n \leq m $, therefore, we have
%$$U_{CP}^N(n)\leq U_{CP}^N(m) \forall n \leq m $$
%Utility of ISP is given as 
%\begin{align*}
%U_{ISP}^{N}&=n\beta^{N}r\log({a^{N}}+1)-nca^N\\
%&=n\left[\beta^{N}r\log({a^{N}}+1)-ca^N\right]\\
%&=n\beta^{N}r\log\left(\frac{\beta^{N}r}{c}\right)-nc\left(\frac{\beta^N r}{c}-1\right)\\
%&=n\beta^{N}r\left(\frac{1-\beta^{N}}{n\beta^N}\right)-n\beta^Nr+nc\\
%&=r+nc-(n+1)\beta^Nr
%\end{align*}
%We can also right Utility of ISP from each CP as
%\begin{equation}
%\beta^{N}r\log({a^{N}}+1)-ca^N
%\end{equation}
%Substituting the value of $a^N=\frac{\beta^Nr}{c}-1$ in the second term, we get
%\begin{align*}
%&\beta^{N}r\log({a^{N}}+1)-c\left(\frac{\beta^Nr}{c}-1\right)\\
%=&	\beta^{N}r\log({a^{N}}+1)-\beta^{N}r+c\\
%=& \beta^{N}r \left(\log({a^{N}}+1)-1\right)+c
%\end{align*}
%\textbf{Since $\beta^N$ ans $a^N$ decreases with increase in $n$, it is clear from above expression that utility of ISP from each CP also decreases with increase in number of CPs.}\\
%
%Now, consider total utility of ISP:
%
%\begin{align*}
%U_{ISP}(n)^N&=r+nc-(n+1)\beta^N(n)r\\
%	=&r+nc-n\beta^N(n)r-\beta^N(n)r
%\end{align*}
%
%as   $n\rightarrow \infty$, $\beta^N(n) \rightarrow \frac{c}{r}$ and $n\beta^N(n)\rightarrow \frac{nc}{r}+1$, so we get:
%\begin{align*}
%	U_{ISP}(n)^N&=r+nc-\left(\frac{nc}{r}+1\right)r-\frac{c}{r}r\\
%	&=-c
%\end{align*}
%Now, $U_{ISP}(n)^N$ increases with increase in $n$ iff
%\begin{align*}
%	\frac{U_{ISP}(n)^N}{\partial n}&>0 \hspace{2mm} \text{(considering $n$ to be continuous)}\\
%	c-\frac{1}{n^2W\left(\frac{r}{nc}e^\frac{1}{n}\right)}&\left(\frac{n^2+n+1-nW\left(\frac{r}{nc}e^\frac{1}{n}\right)}{n\left(1+W\left(\frac{r}{nc}e^\frac{1}{n}\right)\right)}\right)r<0\\
%	\frac{1}{n^2W\left(\frac{r}{nc}e^\frac{1}{n}\right)}&\left(\frac{n^2+n+1-nW\left(\frac{r}{nc}e^\frac{1}{n}\right)}{n\left(1+W\left(\frac{r}{nc}e^\frac{1}{n}\right)\right)}\right)<\frac{c}{r}
%\end{align*}
%Since, $c/r>0$, we have
%$$	\frac{1}{n^2W\left(\frac{r}{nc}e^\frac{1}{n}\right)}\left(\frac{n^2+n+1-nW\left(\frac{r}{nc}e^\frac{1}{n}\right)}{n\left(1+W\left(\frac{r}{nc}e^\frac{1}{n}\right)\right)}\right)<0$$
%$$\iff n^2+n+1-nW\left(\frac{r}{nc}e^\frac{1}{n}\right)<0 $$
%\textbf{Total Utility of ISP first increases with increase in $n$ and after certain value of $n$, it starts falling down, this $n$ is given by following equation for give $r/c$:}
%\begin{equation}
%n^2+n+1=n W\left(\frac{r}{nc}e^\frac{1}{n}\right)
%\end{equation}
%Under the non-neutral regime, the effort levels that optimize the ISP utility for given contracts $\beta_i, i=1,2,...,n$ are:
%$$a_i^*=\max\left(\frac{\beta_ir}{c}-1,0\right) \mbox{ for }  i=1,2,..., n.$$
%Simplified optimization problem for  each $CP_i$ can be expressed as the following: \\
%\begin{align*}
%& \textbf{NonNeutral:}\\
%&\max_{\beta_i \in [0,1]} \hspace{2mm} (1-\beta_i)\log\left(\max\left(\frac{\beta_ir}{c},1\right)\right)r&\\
%%&\hspace{10mm}-\frac{z}{2}[(\beta_1r_1\sigma_1)^2+(\beta_2r_2\sigma_2)^2+2\rho\beta_1\beta_2r_1r_2\sigma_1\sigma_2]\\
%%&\hspace{20mm}\text{where} %\hspace{1.5mm}\overline{h}=-\log (-\overline{H}).
%\end{align*} 
%
%and thus equilibrium effort becomes:
%\begin{equation} \label{eqnNNa}
%a=\max\left(\frac{\beta r}{c}-1,o\right)
%\end{equation}
%Utility of each CP is given as 
%\begin{align*}
%U_{CP}^{NN}&=(1-\beta^{NN})r\log\left(\frac{\beta^{NN}r}{c}\right)\\
%&=(1-\beta^{NN})r\frac{(1-\beta^{NN})}{\beta^{NN}}\\
%&=\frac{(1-\beta^{NN})^2}{\beta^{NN}}r
%\end{align*}
%Utility of ISP is given as 
%\begin{align*}
%U_{ISP}^{NN}&=n\beta^{NN}r\log({a^{NN}}+1)-nca^{NN}\\
%&=n\left[\beta^{NN}r\log({a^{NN}}+1)-ca^{NN}\right]\\
%&=n\beta^{NN}r\log\left(\frac{\beta^{NN}r}{c}\right)-nc\left(\frac{\beta^{NN} r}{c}-1\right)\\
%&=n\beta^{NN}r\left(\frac{1-\beta^{NN}}{\beta^{NN}}\right)-n\beta^{NN}r+nc\\
%&=r+nc-2n\beta^{NN}r
%\end{align*}




==> Journal Version Arxiv/bargaining.tex <==
In this section, we consider the cooperative scenario where CPs in the neutral regime bargain to arrive at an agreement on their revenue share proportions to be given to ISP. We use the classical cooperative solution concept, the Nash Bargaining solution \cite{NBS}.
A Nash Bargaining solution $(\beta_1^B,\beta_2^B)$ is defined as the solution of the following maximization problem:
\begin{align*}
\max_{\beta_1,\beta_2} &\hspace{2mm} (U_{CP_1}-d_{CP_1})(U_{CP_2}-d_{CP_2})\\
&\text{s.t.}\hspace{4mm}(U_{CP_1},U_{CP_1})\in \mathcal{S}\\
&\hspace{4mm} 0 \le\beta_1\le 1,0 \le \beta_2 \le 1
\end{align*}
where $\mathcal{S}$ of the set of all feasible, non-negative utility vectors given by $$\mathcal{S}:=\{(U_{CP_1}(\beta_1,\beta_2),U_{CP_2}(\beta_1,\beta_2))| \hspace{0.5mm}0\leq \beta_1\leq1,0\leq\beta_2\leq 1\} \cap \mathbb{R}^2_+$$
and $d_{CP_i} ; i=1,2$ are disagreement points. In our case, the disagreement points correspond to the utility that the CP$_i$ gets when fails to arrive at an agreement to share revenue proportion with ISP. These are equal to zero ($d_{CP_1}=d_{CP_2}=0$), since when no revenue is shared by CPs, there is no investment (effort) by ISP in the network and utility of each CP is zero.
\subsection{Symmetric case}
In this section, we consider the Nash Bargaining Problem (NBP) between the CPs when they are symmetric with respect to revenue per click rates, i.e., $r_1=r_2=r$. For this case, given ISP investment decision, NBP between CPs is given as follows:
\begin{align*}
\max_{\beta_1,\beta_2} &\hspace{2mm} (1-\beta_1)(1-\beta_2)r^2\left[\log\left(\frac{(\beta_1+\beta_2)r}{2c}\right)\right]^2\\
&\text{s.t.}\hspace{10mm} 0 \le\beta_1\le 1,0 \le \beta_2 \le 1
\end{align*}

\begin{thm} \label{thm:NBS1}
	The NBS of the above NBP is given as:
	$$\beta_1^B=\beta_2^B=\beta^B=\frac{1}{W\left(\frac{r}{c}e\right)}  \hspace{1mm} \forall \frac{r}{c}>1
$$

\end{thm}

%%
\subsection{General case}
In this section, we consider the Nash Bargaining Problem (NBP) between the CPs when they are asymmetric with respect to revenue per click rates, i.e., $r_1\ne r_2$, and without loss of generality we assume that $r_1>r_2$. For this case, given ISP investment decision, NBP between CPs is given as follows:
\begin{align*}
\max_{\beta_1,\beta_2} &\hspace{2mm} (1-\beta_1)(1-\beta_2)r_1r_2\left[\log\left(\frac{\beta_1r_1+\beta_2r_2}{2c}\right)\right]^2\\
&\text{s.t.}\hspace{13mm} 0 \le\beta_1\le 1,0 \le \beta_2 \le 1
\end{align*}

\begin{thm} \label{thm:NBS2}
	The NBS of the above NBP is given as:
	\begin{equation}
(\beta_1^B,\beta_2^B)=\begin{cases}
\overline{\beta}_1^B, \overline{\beta}_2^B &\mbox{  if }  \frac{r_1+r_2}{r_1-r_2} > W\left(\frac{r_1+r_2}{2c}e\right), \\
(\hat{\beta}_1^B,0)  &\mbox{  else }  
\end{cases}
\end{equation}
where
\begin{equation}\nonumber
\overline{\beta}_1^B=\frac{r_1+r_2}{2r_1W\left(\frac{r_1+r_2}{2c}e\right)}-\frac{r_2-r_1}{2r_1}
\end{equation}
\begin{equation} \nonumber
\overline{\beta}_2^B=\frac{r_1+r_2}{2r_2
	W\left(\frac{r_1+r_2}{2c}e\right)}-\frac{r_1-r_2}{2r_2}
\end{equation}
$$
\hat{\beta}_1^B=\frac{2}{
	W\left(\frac{r_1}{c}e^2\right)}
$$
\end{thm}

It is not necessary that disagreement point is $(0,0)$, it is possible when CPs don't agree on the bargaining contract, they may act non-cooperatively and in that case disagreement point is the equilibrium solution of the non-cooperative game between CPs. 
fo
\begin{figure*}[h!] 
	\centering
	{\includegraphics[scale=0.35]{figures/b1}%
	}
	{\includegraphics[scale=0.35]{figures/b2}%
}
	{\includegraphics[scale=0.35]{figures/A}%
}
	{\includegraphics[scale=0.35]{figures/CP1U}%
}
{\includegraphics[scale=0.35]{figures/CP2U}%
}
{\includegraphics[scale=0.35]{figures/ISP}%
}
{\includegraphics[scale=0.35]{figures/ScU}%
}
	\caption {Comparison between Non-neutral, neutral and bargaining setup when CPs are asymmetric when disagreement point is $(0,0)$. We fix $c=1, r_2=2$ and vary $r_1$ from 2 to 30.}
%	\label{fig:comparisonISP}
\end{figure*}

\begin{figure*}[h!] 
	\centering
	{\includegraphics[scale=0.35]{figures/beta1nbs}%
	}
	{\includegraphics[scale=0.35]{figures/beta2nbs}%
	}
	{\includegraphics[scale=0.35]{figures/totaleffortb}%
	}
	{\includegraphics[scale=0.35]{figures/CP1Ub}%
	}
	{\includegraphics[scale=0.35]{figures/CP2Ub}%
	}
	{\includegraphics[scale=0.35]{figures/ISPUb}%
	}
	{\includegraphics[scale=0.35]{figures/SUb}%
	}
	\caption {Comparison between Non-neutral, neutral and bargaining setup when CPs are asymmetric and disagreement point is Nash Equilibrium. We fix $c=1, r_2=2$ and vary $r_1$ from 2 to 10.}
\end{figure*}



%\begin{figure*}[h!] 
%	\centering
%	{\includegraphics[scale=0.35]{figures/CP1U}%
%	}
%	{\includegraphics[scale=0.35]{figures/CP2U}%
%	}
%	{\includegraphics[scale=0.35]{figures/ISP}%
%	}
%	{\includegraphics[scale=0.35]{figures/ScU}%
%}
%	\caption {Comparison between Non-neutral, neutral and bargaining setup when CPs are asymmetric. We fix $c=1, r_2=2$ and vary $r_1$ from 2 to 20.}
%	%	\label{fig:comparisonISP}
%\end{figure*}

==> Journal Version Arxiv/forcing_neutrality.tex <==

Competition between CPs induces non-neutral behavior in separate effort case, i.e. different effort made by the ISP for each CP ($a_1 \neq a_2$). In this case, neutrality can be imposed by making the same effort of the ISP for both CPs equal. We can think about an external control done by an entity (the governmental authority for example). This external entity may impose a tax on the contents such that the resulting investment strategy of the ISP is neutral, i.e. $a^*_1=a^*_2$. We can then think about a three layers hierarchical game where:
\begin{enumerate}
	\item At the higher level (authority level), the authority determines the taxes that each CP$_i$ has to pay on their benefit (for example a percentage of the net profit, say $t_i$) in order to minimize the difference between $a_1^*$ and $a_2^*$.
	\item At the intermediate level, based on this tax, each CP $i$ determines the optimal contract $s_i(.)$ with the ISP.
	\item Finally, at the lower level, the ISP determines optimally his investment $a_i$ for each CP$_i$ traffic.
\end{enumerate}
The problem for CP$_i$ is give as
\begin{align*}
&\hspace{10mm}\max_{a_1, a_2 \beta_i} \hspace{2mm} (1-\beta_i)(1-t_i)r_i\log(a+1)\\
&\text{s.t.}\\
&\text{argmax}_{a_1,a_2}\hspace{3mm} \sum_iz\left(\beta_i(1-t_i)r_i\log(a_i+1)-ca_i\right)
\end{align*}
\begin{lemma}
	The action by ISP for each $CP_i$ is given by\\ 
	%$$
	%\beta_1^*=\frac{c(a_1^*+a_2^*)}{r_1P_1}, \beta_2=\frac{c(a_1^*+a_2^*)}{r_2P_2}
	%$$
	\begin{equation}
	a_i+1=\max\left(\frac{\beta_ir_i(1-t_i)}{c},1\right) , i=1,2
	\end{equation}
\end{lemma}
\begin{lemma}
	The equilibrium solution of the above problem is given as:
	\begin{equation}
		(\beta_1^*,\beta_2^*)=\begin{cases}
		0  &\mbox{  if }  \frac{r_i(1-t_i)}{c}\leq 1 \forall i=1,2, \\
		\left(\frac{1}{W\left(\frac{r_1(1-t_1)}{c}e\right)}, 0\right)  &\mbox{  if }  \frac{r_1(1-t_1)}{c} > 1, \frac{r_2(1-t_2)}{c} \le 1 
		\\
		\left(0, \frac{1}{W\left(\frac{r_2(1-t_2)}{c}e\right)}\right)  &\mbox{  if }  \frac{r_1(1-t_1)}{c} \le 1, \frac{r_2(1-t_2)}{c} > 1 
		\\
		\left(\frac{1}{W\left(\frac{r_1(1-t_1)}{c}e\right)}, \frac{1}{W\left(\frac{r_2(1-t_2)}{c}e\right)}\right)  &\mbox{  if }  \frac{r_1(1-t_1)}{c}>1,  \frac{r_2(1-t_2)}{c}>1 
	\end{cases}
	\end{equation}
\end{lemma}
\begin{lemma}
	The tax $t_i$ for each CP$_i; i=1,2$ is imposed s.t.
	$$e^{W\left(\frac{r_2(1-t_2)}{c}e\right)-W\left(\frac{r_1(1-t_1)}{c}e\right)}=\frac{r_2}{r_1}   $$
\end{lemma}

==> Journal Version Arxiv/general.tex <==

In this subsection we compare the contracts, utilities of the CPs and the
ISP, and the social utility at equilibrium obtained under the neutral
and the non-neutral regime. We focus on the case of $n=2$ for comparing the non-neutral and neutral regime. Without loss of generality, we assume $r_1 \geq r_2$, i.e.,
$\mbox{CP}_1$ earns higher per unit demand than $\mbox{CP}_2$. We
refer to $\mbox{CP}_1$ as the dominant CP and $\mbox{CP}_2$ as the
non-dominant CP. \textcolor{red}{This constraint will be considered for the rest of
the paper.} What does this line mean?
%We begin with the non-neutral regime. 

%\subsection{Non-neutral regime}
%Under the non-neutral regime, it is easy to see that when
%$\overline{H}=-1$, the CP decisions are no more coupled. The
%optimization problem for $CP_i, i=1,2$ simplifies to:
%\begin{align*}
%&\max_{\beta_i\in [0,1]} \hspace{2mm} (1-\beta_i)r_i\log\left(\max\left(\frac{\beta_ir_i}{c}-1,0\right)+1\right).
%\end{align*}
%Let  $W(\cdot)$ denote the stand LambertW function \textcolor{blue}{\cite{}} taking values on the principle branch. The optimal contract is characterized in term LambertW function in the following. %Each CP has his own constraint optimization problem with common constraint which is the optimization problem of the ISP. Then, the global problem can be seen as a hierarchical non-cooperative game between CPs (here 2 leaders) and one ISP (one follower).Usually, this type of complex game involves the framework of Generalized Nash Equilibrium Point (GNEP) and tools from it mainly for optimization theory and KKT conditions. In our setting, we are able to determine explicitly the equilibrium solution of this hierarchical game between two CPs and one ISP.

\begin{cor}
\label{cor:NN-asy}
In the non-neutral regime, $\CPi, i=1, 2,$ shares a positive fraction
of the revenue at equilibrium with the ISP if and only if $r_i/c
>1$. Specifically, the equilibrium contract is as follows (recall that
$r_1 \geq r_2)$:
	\begin{equation}
(\beta_1^*,\beta_2^*)=\begin{cases}
(0,0)  &\mbox{  if }  \frac{r_i}{c}\leq 1 \forall i=1,2, \\
\left(\frac{1}{W\left(\frac{r_1}{c}e\right)}, 0\right)  &\mbox{  if }  \frac{r_1}{c} > 1, \frac{r_2}{c} \le 1, 
%\\
%\left(0, \frac{1}{W\left(\frac{r_2}{c}e\right)}\right)  &\mbox{  if }  \frac{r_%1}{c} \le 1, \frac{r_2}{c} > 1, 
\\
\left(\frac{1}{W\left(\frac{r_1}{c}e\right)}, \frac{1}{W\left(\frac{r_2}{c}e\right)}\right)  &\mbox{  if }  \frac{r_1}{c}>1,  \frac{r_2}{c}>1,
\end{cases}
\end{equation}	
where $W(\cdot)$ denotes the standard LambertW function \cite{corless1996lambertw}.
\end{cor}
\noindent
Notice that if $r_i$ increases, $\beta_i^*$ decreases, i.e., $\CPi$
shares a small fraction of its revenue with the ISP.
\textcolor{red}{This is because if a CP's capability to translate its demand to
earning improves, then it may require less effort from the ISP to
improve demand for its content and hence can reduce the incentives it
gives through revenue-sharing.}
\textbf{JK: Not obvious here that decreasing $\beta$ implies decreasing
effort! (see the first equation on this column)}


%\subsection{Neutral Regime}
%In the neutral regime, ISP is forced to make the same investment
%decision for both CPs, i.e., $a_1=a_2=a$. The optimization problem for
%CP $i$ in this case simplifies to:
%\begin{align*}
%&\max_{\beta_i \in [0,1]} \hspace{2mm} (1-\beta_i)\log\left(\max\left(\frac{\beta_1r_1+\beta_2r_2}{2c}-1,0\right)+1\right)r_i.
%\end{align*} 
The following theorem gives  equilibrium contracts at equilibrium in the neutral regime for two CPs..

\begin{thm} \label{Thm:Neutral-asym}
Let $r_1 \geq r_2$ and $\frac{r_i}{c} > 1$ for all $i$. If
	$\frac{r_1}{2c}>1,$ then the equilibrium contract in the
	neutral regime is given by:\\ \begin{equation}
	(\beta_1^*,\beta_2^*)=\begin{cases}
	(\overline{\beta}_1, \overline{\beta}_2) &\mbox{ if
	} \frac{r_1+r_2}{r_1-r_2} >
	2W\left(\frac{r_1+r_2}{4c}\sqrt{e}\right), \\ \left(\frac{1}{
	W\left(\frac{r_1}{2c}e\right)},0\right) &\mbox{
	otherwise}, \end{cases} \label{eqn:NeutralConds} \end{equation}
	where \begin{equation}\nonumber \overline{\beta}_1=\frac{r_1+r_2}{4r_1W\left(\frac{r_1+r_2}{4c}\sqrt{e}\right)}-\frac{r_2-r_1}{2r_1}, \overline{\beta}_2=\frac{r_1+r_2}{4r_2
	W\left(\frac{r_1+r_2}{4c}\sqrt{e}\right)}-\frac{r_1-r_2}{2r_2}.  \end{equation}
	Otherwise, the equilibrium contract is
	$(\beta_1^*,\beta_2^*)=(0,0)$, i.e., none of the CPs will
	share their revenue with the ISP.
\end{thm}
In the following we use the notation $(\beta_1^N, \beta_2^N)$ and $(\beta_1^{NN}, \beta_2^{NN})$ to denote the equilibrium contract profiles in the neutral and non-neutral regimes, respectively. Further, we superscript all quantities evaluated under the neutral regime by $N$ and those computed under non-neutral regime by $NN$. For notational convenience let $r_1^*:=r_1^*(r_2)$ denote the value of $r_1$ that satisfies the following relation for a given $r_2$
$$\frac{r_1+r_2}{r_1-r_2} = 2W\left(\frac{r_1+r_2}{4c}\sqrt{e}\right).$$
For $r_1\leq r_1^*$ the first condition in (\ref{eqn:NeutralConds}) is satisfied where revenue shared by  both the CPs is strictly positive, i.e., $\beta_i^{N}>0$ for all $i=1,2$. For $r_1 > r_1^*$ the second condition holds in which only the $\mbox{CP}_1$'s share is strictly positive and $\mbox{CP}_2$ does not share anything, i.e., $\beta_1^N>0$ and $\beta_2^N=0$. Further, it is easy to verify that $r_1^*$ is monotonically increasing in $r_2$ and $r_1^*>  r_2$.
%The above theorem gives equilibrium of the game between CPs under the assumption that $\frac{r_i}{c} > 1 \forall i=1,2$, $\frac{r_i}{2c}>1$ for at least one $i$. 


==> Journal Version Arxiv/introduction.tex <==

The rapid growth of data-intensive services has resulted in an explosion of the Internet traffic, and it is expected to increase at an even faster rate in the future \cite{jung2011cisco}. 
%This has caused serious network congestion, especially in wireless
%networks which are bandwidth constrained.
To accommodate this increase in traffic, and to provide better Quality of Service (QoS) for end users, Internet service providers (ISPs) need to upgrade their network infrastructure and expand capacity. This development follows the deployment of next generation networks that will induce more business interactions between service providers and content providers. For example, caching technologies has recently received increased attention from industry and academia to be a key solution for next generation networks \cite{Paschos2018jsac}. As it is specified in this special issue, the economics of caching will be one of important aspect in deciding the monetary interactions between the ISPs and CPs.


In terms of return on investments, the ISPs, especially the ones providing last-mile connectivity, feel that the revenue from end-users (mainly access charges) are often not enough to recoup their investment costs and they propose that the CPs share the risk by sharing part of their revenues. The CPs may also have the incentive to contribute to ISP capacity expansion, as increased capacity and better QoS trigger higher demand for content and help them earn even higher revenues (mainly from subscriptions and advertisements) \cite{sen2013survey}. For example, in \cite{Krolikowski2018jsac}, the authors propose a model in which a Mobile  Network  Operator  leases its  edge caches to  a Content Provider. This is an increasingly relevant scenario and follows proposals for deploying edge storage resources at mobile 5G networks \cite{Bastug2014ieeemag}. A recent announcement by Comcast that it will bundle Netflix subscription in its package is another example of an ISP helping a CP to increase its demand.


%{\bf Now connect here to the Moral Hazard problem}
%Both CP and ISP engage in risk sharing under conditions such that their privately taken action of ISP (investment) affect the probability distribution of the outcome for CP (demand).as CP will incur the cost by sharing its revenue.

%ISP gets involved in a risky situation as its investment cost may not be recovered from customers access fees and therefore seek protection against the risk from the CPs. On the other hand, CPs would like the ISPs to take the risk of investing into the network infrastructure as they would benefit from ISPs investments and may like to share the risk by giving them part of their earning. %The CPs would be willing to give the ISPs in proportion to the benefit they derive from the increased traffic in the Internet which in turn depends on the ISP investments. 
%However, the CPs may not be able to directly observe the investments of the ISPs, but can estimate its thorough the increase in demand for their contents. This is the classical  moral hazard situation between principle and agent where a CP acts as a principal and an ISP acts as an agent \cite{b8}. However, the classical moral hazard problem deals with a single principle and an agent, whereas we are faced with possibly multiple principles and agents. In this work, we focus on a monopolistic ISP connecting end users to multiple CPs i.e., multiple principles and a single agent. Our interest is in determining optimal sharing mechanisms/contracts between each CP and the ISP.

If a CP enters into a contract with an ISP to share its revenue in return for ISP putting efforts to improve demand for its content, the CP may want to monitor the efforts level of ISP so that the contract is honored.  However such monitoring of efforts levels may not be always feasible in the Internet as there is an inherent asymmetry of information between CPs and ISPs -- CPs cannot observe the exact investment (caching effort) made by the ISP, but can only observe the resulting increase in user demand for its content, which is a (random) function of the ISP's investment. In this situation, an obvious question arises: how can this imperfect information about the ISP's investment be used to formulate an optimal revenue sharing contract?  This is a situation where a privately taken action (investment) by the ISP influences the probability distribution of the outcome (demand) for the CP.
%This leads to problem of moral hazard as principal (CP) and agent
%(ISP) get involve in risk sharing situation through a contract and
%there is asymmetry of information.


The role of this information asymmetry between the CP and ISP is critical under such agreements, where ISP makes an investment which ultimately benefits the CP, and should be considered in the structure of the contract. Therefore, moral hazard can be applied to propose a contract in which the ISP (agent) knows that CP (principle) will pay to cover its risks, which in turn gives the ISP the incentive to make the (risky) investment. Also, the moral hazard model is proven to induce proper incentives for taking appropriate action \cite{holmstrom1979moral}, and this may provide fair revenue sharing between CPs and ISPs.  In our work, we propose an incentivizing mechanism using the \textit{moral hazard} approach in which CPs share a part of their revenues with an ISP expecting a better QoS for their content and higher revenue in return from the ISP efforts.
%One the other hand, CPs can observe the growth in revenues due to
%higher traffic . This disparity, has created net-neutrality debate as
%ISPs have proposed that CPs return the benefit of value chain by
%sharing their revenues with them. The ISP does not reveal exact
%investment cost incurred, however, CP's demand is affected by ISP's
%investment in the network, which can be estimated with some
%probability distribution by CP. This creates the problem of moral
%hazard, since privately taken action (investment) of ISP affects the
%probability distribution of the outcome (demand) for CP . Under such
%situation, the question arises is "what should be the fare share of
%revenue between CP and ISP?"


The classical moral hazard problem deals with a single principle and a single agent, whereas we are faced with possibility of multiple principles interacting with multiple agents. In this work, we focus on a monopolistic ISP connecting end users to multiple CPs, i.e., multiple principles and a single agent. Our interest is in determining optimal sharing mechanisms/contracts between each CP and the ISP. We distinguish two cases for the effort (investment) made by the ISP. In one case, we allow the ISP to make different amounts of effort for each CP, and in the other case, the ISP is constrained to put an equal amount of effort for all CPs. The former case corresponds to a `non-neutral' regime where the ISP is allowed to differentiate between CPs, and the latter case corresponds to a `neutral' regime where the ISP cannot differentiate between CPs. We compare the revenue of each players and social utilities under both the regimes and analyze which regime is preferred by the players. 

We consider competition between multiple CPs that provide content of a
particular type, for example, video, and aim to earn higher revenue by
entering into a revenue sharing contract with the ISP. Each CP
separately negotiates with the ISP knowing that the other CPs can also
enter into similar negotiations with the ISP. We consider linear contracts and analyze the
equilibrium sharing contracts in both the neutral and non-neutral
regime. We first consider the symmetric case where all the CPs earn same revenue per unit demand. This corresponds to the case where ability of the CPs to monitize their demand is the same. We then study the asymetric case where the CPs capability to monetize their demand could be different. Our
contributions and observations can be summarized as follows:
\begin{itemize}
\item We model the competitive revenue sharing of CPs with an ISP in return for improved QoS in the moral hazard framework with multiple principles and a single agent.
\item We analyze the equilibrium contracts in a regime where the ISP
can put a different level of effort for each CP (non-neutral) and in a
regime where it is constrained to put equal efforts for all CPs
(neutral).
\item In the symmetric case we show that all the players prefer the non-neutral regimes as their utilities are higher
\item In the asymmetric case we show that the CP which can better monetize the demand for
its traffic always prefers the non-neutral regime whereas the CP with weaker monetization power can prefer the neutral or non-neutral regime depending on its relative monetization power.
\item The ISP always prefers the non-neutral regime. Moreover,
social utility (defined as the sum of the average earning of all
players) is also higher in the non-neutral regime.
\end{itemize}

This paper is organized as follows. In Section~\ref{sec:problem} we
discuss the problem setup and define contracts under the neutral and non-neutral regime. We study the equilibrium contracts under neutral and non-neutral regime under the symmetric case in in Section~\ref{sec:MultipleSymmetric} and under asymetric case in Section~\ref{sec:AsymetricCase}. Conclusions and future extensions are discussed in Section~\ref{sec:Conlcusion}. Proofs of all stated results can be
found in the appendix.

\subsection{Related works}
Several works \cite{kamiyama2014effect, kamiyama2014feasibility,
park2014isp1, park2014isp2, im2016revenue} study the possibility of
content charges by ISPs to recover investment
costs. In \cite{kamiyama2014effect}
and \cite{kamiyama2014feasibility}, the authors investigated the
feasibility of ISPs charging a content charge to CPs, and evaluate its
effect by modeling the Stackelberg game between CPs and
ISPs. In \cite{park2014isp1} and \cite{park2014isp2}, a revenue-sharing scheme is proposed when the ISP provides a content piracy
monitoring service to CPs for increasing the demand for their content.
This work is extended to two ISPs competing with each other
in \cite{im2016revenue} where only one of them provides the content
piracy monitoring service. Several studies considered
cooperative settlement between service providers for profit
sharing \cite{ma2010,ma2011,yeze2017} where the mechanisms are derived
using the Shapely value concept.


%Later in \cite{ma2011}, they extended the model for three classes of
%ISPs: content, transit, and eyeball. Then, in \cite{yeze2017} authors
%used the concept of caching game between CPs and ISPs, where ISP
%deploy cache for CP, where sharing of profit earned by CP and the
%cache cost incurred by ISP is given by Shapely value.  While the rest
%of the studies neglected the issue of moral hazard in revenue sharing
%between CP and ISP.

A moral hazard framework is applied in \cite{constantiou2001information} to study interconnection contracts between ISP and end users in the market for network transport services. However, the contract design problem between ISPs and CPs remained unaddressed in this work. In the present paper, we apply the moral hazard approach to study revenue sharing between an ISP and multiple CPs. The CPs act as the principles that enter into a contract with the ISP (agent) to improve QoS for their content. We thus end up with a multiple principle, single agent problem.
%Under the contract, ISP has to make some investment decision which impacts the demand for CPs. 
%In our setting, a shared constraint game known as Generalized Nash Equilibrium Problem (GNEP) is formulated where both competing CPs share common constraints. A regulator may play an important role in the system, particularly to enforce the ISP to invest in the network infrastructure for the benefit of both CP traffic (to be neutral). This comes from the weak performance of the system because of the asymmetries information of the principal-agent problem as stated in \cite{Jamison16}. Therefore, such regulatory intervention is considered in the last section of our problem. 

A moral hazard framework where two principals offer a contract to the same agent is studied in \cite{commonagency} where the principals can only observe correlated noisy signals of the common one-dimensional action taken by the agent, where the principals' output is linearly increasing with the agent's action. Our work is different from them as we consider that even though the agent (ISP) is common, it chooses different actions for each principal (CP). We also compare it with the setting when the ISP is forced to choose the same action for both CPs.  Also, we consider the demands of CPs to be logarithmic in the efforts of the agent, unlike the linear case considered in \cite{commonagency}. Such a demand function comes from the fact that the delay experienced by end users is exponential in the cache and not linear as assumed in \cite{yeze2017} and \cite{kesidis13}.

A moral hazard setup is also used in \cite{Zhang17} for motivating end users to participate in crowd-sourced services in one principal and several agent problem.  %Moral hazard problems are basically analyzed considering Bayesian equilibrium solution and Stackelberg approach. In fact, the principal has an equivalent role of leader and the agent of the follower. Therefore, techniques inspired from bilevel programming can be used to study equilibrium solutions \cite{colson05}. In our work, we focus on the special case where the shared constraint on ISP's utility is always satisfied, so apply standard backward induction technique used in Stackelberg games.




%In \cite{b5} authors considered two sided market in which they studied the revenue sharing between ISP and CP through collaboration where ISP applies effort to reduce online content piracy. They formulated a sequential game between ISP and CP, where ISP controls content piracy factor and CP controls price to end users and discussed different sharing schemes. Then, cooperative game between CP and ISP is studied in \cite{b6} in which revenue sharing factor is negotiated between them. Users’ demand is determined by hoteling model. Both CP and ISP then maximizes their revenue to determine s traffic monitoring rate and content price respectively. Given fixed revenue sharing factor, best response of CP and ISP is calculated. 




==> Journal Version Arxiv/linear.tex <==
In this section, we consider special case that $CP_i$ offers a linear contract to ISP of the form $s_i(X_i)=\beta_i X_i$ and ISP chooses whether to accept or reject the contract. Note that linear contracts have been shown to be optimal in \cite{Holmstrom1} particularly when agent has a risk averse utility as it is our case in our setting. In fact, if ISP accepts the contract, he chooses an action (a caching effort) $a_i\in A\equiv [0,\infty]$ for each  $CP_i$. ISP rejects the contract if he gets expected utility below a reserve utility denoted by $\overline{H}$. ISP has constant absolute risk aversion (CARA) utility as $H(W)=-e^{-zW}$, where $W$ is wealth and $z>0$ is a fixed constant. CP$_i$ observes a demand, that depends on caching effort $a_i$ by the ISP, and estimates it as a random variable
$D_i:=\log(a_i+1)+\epsilon_i$,  where $\epsilon_i$ is a random error observed for the demand for content of CP$_i$. Each $\epsilon_i $ is assumed to be Gaussian distributed with mean $0$. Random errors are not independent and the covariance matrix $K$ is given by: \[
K =
\left[ {\begin{array}{cc}
	\sigma_1^2 & \rho \sigma_1\sigma_2 \\
	\rho \sigma_1\sigma_2 & \sigma_2^2  \\
	\end{array} } \right].
\]
The total revenue generated for CP$_i$ due to his demand is $X_i=r_iD_i$ where $r_i$ is the revenue per click for $CP_i$ when $D_i$ is, for example, associated to a number of clicks. Each CP$_i$ is assumed to be risk neutral with a utility function expressed as $V_i(X-s_i(X))=X-s_i(X)$. Cost incurred by ISP is assumed to be increasing in the global caching effort as $c(a_1,a_2)=c(a_1+a_2)$.
% Here, caching cost is different for each CP because we assume that each CP provide  different type of contents.
The expected utility of $CP_i$ is given by:
\begin{align*}
E[V(X_i-s_i(X_i))]&=E[V(X_i-(\beta_i X_i))],\\
& =E[X_i(1-\beta_i)]=(1-\beta_i)r_i\log(a_i+1),
\end{align*}
%\begin{eqnarray}\nonumber 
%&E[V(X_i-s_i(X_i))]=E[V(X_i-(\alpha_i+\beta_i X_i))]&\\
%& =E[X_i(1-\beta_i)-\alpha_i] =(1-\beta_i)r_i\log(a_i+1)-\alpha
%_i,&
%\end{eqnarray}
and the expected utility of $ISP$ is given by:
\begin{align*}
E[H(\sum_i[s_i(X_i)-ca_i])]&=E[H(\sum_i[\beta_ir_i(\log(a_i+1)+\epsilon_i)-ca_i])]\\
&=E[-\exp\sum_i[\beta_ir_i(\log(a_i+1)+\epsilon_i)-ca_i]]\\
&=-\exp\{-z\sum_i[\beta_ir_i\log(a_i+1)-ca_i]\\
+\frac{z^2}{2}[(\beta_1r_1\sigma_1)^2+&(\beta_2r_2\sigma_2)^2+2\rho\beta_1\beta_2r_1r_2\sigma_1\sigma_2]\}.
\end{align*}
The expression for the ISP expected utility follows after noting that it is the characteristic function of a Gaussian random vector. ISP's optimization problem is to find an effort level $a_i$ for each CP$_i$ which maximizes its expected utility. Maximizing expected utility over both $a_i$ is equivalent to maximizing its negative exponent term.
%, i.e.,
%$$
%\sum_i[\beta_ir_i\log(a_i+1)-ca_i]-\frac{z}{2}[(\beta_1r_1\sigma_1)^2+(\beta_2r_2\sigma_2)^2+2\rho\beta_1\beta_2r_1r_2\sigma_1\sigma_2]
%$$\\
%\noindent
Therefore, the simplified optimization problem for each $CP_i$, taking into account the ISP optimization problem, is given as the following bilevel optimization problem: 
\begin{align*}
&\hspace{12mm}\max_{a_i, \beta_i} \hspace{2mm} (1-\beta_i)\log(a_i+1)r_i&\\
&\hspace{6mm}\text{s.t.} \hspace{5mm}\sum_i[\beta_ir_i\log(a_i+1)-ca_i]\\
&\hspace{10mm}-\frac{z}{2}[(\beta_1r_1\sigma_1)^2+(\beta_2r_2\sigma_2)^2+2\rho\beta_1\beta_2r_1r_2\sigma_1\sigma_2]\geq \overline{h}\\&
\text{argmax}_{a_1,a_2} \sum_i[\beta_ir_i\log(a_i+1)-ca_i]\\
&\hspace{10mm}-\frac{z}{2}[(\beta_1r_1\sigma_1)^2+(\beta_2r_2\sigma_2)^2+2\rho\beta_1\beta_2r_1r_2\sigma_1\sigma_2]\\
&\hspace{20mm}\text{where} \hspace{1.5mm}\overline{h}=-\log (-\overline{H}).
\end{align*} 
%\begin{eqnarray}
%\nonumber&\max_{a_i, \alpha_i,\beta_i} \hspace{2mm} (1-\beta_i)\log(a+1)r_i-\alpha_i&\\\nonumber \noindent
%&\text{s.t.}\sum_i[\beta_ir_i\log(a_i+1)-ca_i]\\
%&-\frac{z}{2}[(\beta_1r_1\sigma_1)^2+(\beta_2r_2\sigma_2)^2+2\rho\beta_1\beta_2r_1r_2\sigma_1\sigma_2]\geq \overline{h}&\\ \nonumber
%&\text{argmax}_{a_1,a_2} \sum_i[\beta_ir_i\log(a_i+1)-ca_i]-\frac{z}{2}[(\beta_1r_1\sigma_1)^2+(\beta_2r_2\sigma_2)^2+2\rho\beta_1\beta_2r_1r_2\sigma_1\sigma_2]&\\ \nonumber \noindent
%&\text{where} \hspace{1.5mm}\overline{h}=-\log (-\overline{H})&
%\end{eqnarray}
The lower-level optimization problem, i.e. the ISP effort optimization problem, as the following solution depending on contracts proposed by both CPs.
\begin{lemma}
	The optimal ISP effort level $a_i^*$ for each CP$_i$ is given by
	$$a_i^*=\max\left(\frac{\beta_ir_i}{c}-1,0\right); i=1,2$$
\end{lemma}
%\begin{lemma}
%	There exist continuum of equilibrium $(\beta_1^*,\beta_2^*)$ of the game between CPs satisfying following equality:
%	\begin{align*}
%	&\hspace{2cm}\sum_i[\beta_i^*r_i\log\left(\frac{\beta_i^*r_i}{c}\right)-\beta_i^*r_i]\\
%	&-\frac{z}{2}[(\beta_1^*r_1\sigma_1)^2+(\beta_2^*r_2\sigma_2)^2+2\rho\beta_1^*\beta_2^*r_1r_2\sigma_1\sigma_2]=\overline{h}
%	\end{align*}
	
%\end{lemma}
An important assumption is that the ISP will accept the CP$_i$ contract if and only if his expected net utility $E(s_i(X_i)-ca_i)$ obtained from CP$_i$ is positive. Hence, if $\sum_i[s_i(X_i)-ca_i]) \geq 0$, the ISP will accept both contracts. Considering this natural case (other case is not of interest here as there is only one CP and then no game between several CPs), yields that for all risk averse parameter $z$, the ISP utility $H(W)\geq -1$ and a natural minimum expected utility is $\overline{H}:=-1$. 

%Then, under this assumption on the minimum expected utility level, the ISP will accept both contracts and there exists a unique equilibrium for the non-cooperative game between CP. This game is studied in the following section.


%Now, $-1 \leq \overline{H}\leq 0$ i.e.,   $0\leq \overline{h}<\infty$, and for $\overline{H}>-1 (\overline{h}>0)$, there could exist continuum of equilibrium of the game between CPs s.t. participation constraint is satisfied at equality. For the uniqueness of the equilibrium we need to assume that $\overline{H}=-1 (\overline{h}=0)$, as under this assumption participation constraint will always be satisfied. The uniqueness of the equilibrium of the non-cooperative game between CPs (at upper level) will allow us to compare the neutral and non-nuetral regime. Non-neutral being the one where ISP is allowed to chooses different caching decision $(a_i)$ for each CP$_i$ and neutral being the case where ISP is restricted to take same caching decision $(a_1=a_2=a)$ for each CP. 


%$r_1/r_2$, $\rho$ and $c$ on Social Utility when ISP applies common and separate efforts for CP respectively. We set parameters $r_1=20$, $P_1=P2=1$, $\sigma_1=\sigma_2=0.25$ and $\overline{H}=200$. We set $c_1=c_2=c/2$, in Fig.~\ref{fig:Utility1}, $r_2=15$ in Fig.~\ref{fig:Utility2} and $c_1=1.5$ and $c_2=1$. in Fig.~\ref{fig:Utility3}.
%Maximizng expected utility over $a$ given is equivalent to maximizing following\\
%$
%\alpha_1+\alpha_2+(\beta_1r_1P_1+\beta_2r_2P_2)a-\frac{ca^2}{2}-\frac{r}{2}((\beta_1r_1P_1\sigma_1)^2+(\beta_2r_2P_2\sigma_2)^2+2\rho\beta_1\beta_2r_1P_1r_2P_2\sigma_1\sigma_2)
%$\\
%Now, each CP solves his maximization problem subject to common constraints and $CP_i$ solves:
%Proposition 3 gives equilibrium behavior of CPs and ISP. Here also $\beta_i^*$ takes unique value at equilibrium and CPs set $\alpha_i^*\text{s}$ in such a way that they extract all the surplus from ISP and ISP will only get his reserve utility. There is continuum of equilibria for this game. ISP does not differentiate between CPs. $\beta_i^*$ is increasing in $r_iP_i$. Also, decreasing in $r_jP_j$ for $\rho>0$ and is increasing in $r_jP_j$ for $\rho<0$ (similar to seperate effort case). The benefit by effort of ISP is shared, however, an increase in $r_iP_i$ increases the marginal benefit of $CP_i$ from the effort exerted by the ISP. 

% \begin{figure}[h!]
%	\begin{center}
%		\includegraphics[scale=0.5]{figures/Fig2.png}
%		\caption{\textit{Effect of disparity between revenue per click rates of CPs on Social Utility.}. }
%	\end{center}
%	\label{fig:figure2 }
%\end{figure}

 
% \begin{figure}[h!]
%	\begin{center}
%		\includegraphics[scale=0.5]{figures/Fig3.png}
%		\caption{\textit{Effect of correlation coefficient on Social Utility.}We set parameters $c_1=c_2=c/2$, $r_1=20$,$r_2=15$ $P_1=P2=1$, $\sigma_1=\sigma_2=0.25$, and $\overline{H}=200$. }
%	\end{center}
%	\label{fig:figure2 }
%\end{figure}


%From figure 2, it can be seen that as the difference between $r_1$ and $r_2$ is higher, disparity is higher in case of seperate Effort. Clearly it implies that seperate effort increases asymmetry in the between CPs in the network.


%Expected Utility of $CP_i$ at equilibrium:
%
%$$
%E[V_i]=(1-\beta_i^*)r_iP_ia^*-\alpha_i^*=(1-\beta_i^*)r_iP_i\frac{\beta_1^*r_1P_1+\beta_2^*r_2P_2}{c}^*-\alpha_i^*$$
%=(1-\frac{(1+rc\sigma_2^2)-(\frac{r_2P_2}{r_1P_1})rc\rho \sigma_1 \sigma_2}{(1+rc\sigma_1^2)(1+rc\sigma_2^2)-\rho^2 r^2 c^2 \sigma_1^2 \sigma_2^2})r_iP_i\frac{r_1P_1[1+rc(\sigma_2^2-\rho\sigma_1\sigma_2)]+r_2P_2[1+rc(\sigma_1^2-\rho\sigma_1\sigma_2)]}{(1+rc\sigma_1^2)(1+rc\sigma_2^2)-\rho^2 r^2 c^2 \sigma_1^2 \sigma_2^2}-\alpha_1

%\section{Forcing neutral behavior}
%Competition between CPs induces non-neutral behavior in separate effort case, i.e. different effort made by the ISP for each CP ($a_1 \neq a_2$). In this case, neutrality can be imposed by making the same effort of the ISP for both CPs equal. We can think about an external control done by an entity (the governmental authority for example). This external entity may impose a tax on the contents such that the resulting investment strategy of the ISP is neutral, i.e. $a^*_1=a^*_2$. We can then think about a three layers hierarchical game where:
%\begin{enumerate}
%	\item At the higher level (authority level), the authority determines the taxes that each CP has to pay on their benefit (for example a percentage of the net profit) in order to minimize the difference between $a_1^*$ and $a_2^*$.
%	\item At the intermediate level, based on this tax, each CP $i$ determines the optimal contract $S_i(.)$ with the ISP.
%	\item Finally, at the lower level, the ISP determines optimally his investment $a_i$ for each CP $i$ traffic.
%\end{enumerate}
%When the tax $t_i$ is imposed on the revenue generated by $CP_i$, new revenue becomes $(1-t_i)X_i$.\\
%Equilibrium Solution for new $X_i$:
%$$
%a_1^*=\frac{r_1P_1(1-t_1)(1+rcA)-r_2P_2(1-t_2)rcA}{c[1+2rcA]}
%$$
%$$
%a_2^*=\frac{r_2P_2(1-t_2)(1+rcA)-r_1P_1(1-t_1)rcA}{c[1+2rcA]}
%$$
%$$
%\beta_1^*=\frac{c(a_1^*+a_2^*)}{r_1P_1(1-t_1)}, \beta_2=\frac{c(a_1^*+a_2^*)}{r_2P_2(1-t_2)}
%$$
%$$
%\beta_1^*=\frac{r_1P_1(1-t_1)+r_2P_2(1-t_2)}{r_1P_1(1-t_1)[1+2rcA]}
%$$
%$$
%\beta_2^*=\frac{r_1P_1(1-t_1)+r_2P_2(1-t_2)}{r_2P_2(1-t_2)[1+2rcA]}
%$$\\
%where $A=\sigma_1^2+\sigma_2^2+2\rho\sigma_1\sigma_2$.\\
%To make $a_1^*=a_2^*$, taxes imposed should be according to following equation:
%$$
%\frac{1-t_1}{1-t_2}=\frac{r_2P_2}{r_1P_1\label{den}}
%$$
%(this comes from equating the expressions obtained form $a_1^*$ and $a_2^*$)
%
%\begin{figure}[h!]
%	\begin{center}
%		\includegraphics[scale=0.35]{figures/fig3levels.pdf}
%		\caption{Global interaction system between authority, content providers and the service provider.}
%	\end{center}
%	\label{fig:figure2 }
%\end{figure}


==> Journal Version Arxiv/model.tex <==
 The ISP is risk-averse
and chooses, for each CP $i$, an effort level $a_i$ that benefits the CP$_i$ under the contract. ISP will accept the contract with CP$_i$ only if it gets at least reserve utility denoted $\overline{H}$. CPs observe only a noisy
signal of the effort level chosen by the ISP. Let $X_i$ denote the revenue generated by CP$_i$ and $s_i(X_i)$ denote the share of $X_i$ that goes to the ISP under the contract.  Let $V_i(\cdot)\in\mathbb{R}_+$ denotes the utility associated to the revenue generated by CP$_i$ and it is a function of the net revenue of the CP$_i$, i.e., $X_i -s(X_i)$. This function $V_i(.)$ is typically increasing concave function.The utility of the ISP is a function $H(s_1(X_1),s_2(X_2), a_1,a_2)\in\mathbb{R}_+$. We assume that this function is increasing in $s_i(X_i)$ and decreasing in $a_i$.
%In this section, we analyze a game between two CPs which offer contract to common ISP, under which ISP chooses an effort level $a$ that benefits both CPs. ISP is risk averse and will accept the contract only if it gets at least reserve utility say $\overline{H}$.  
% Let $V_i(\cdot)\in\mathbb{R}_+$ denotes the utility associated to the revenue generated by $CP_i$. For each $X_1$, $X_2$, $s_1(X_1)$, $s_2(X_2)$ and $a$, $H(s_1(X_1),s_2(X_2),a)\in\mathbb{R}_+$ denote the utility of the ISP. We assume that $H(\cdot)$ is increasing in $s_i(X_i)$ and decreasing in $a$.
%$$\frac{\partial H(s_1(X_1),s_2(X_2),a)}{\partial s_i(X_i)}>0, $$
%$$\frac{\partial H}{\partial a_i}(s_1(X_1),s_2(X_2),a)<0. $$

 We further assume that $H(s_1(X_1),s_2(X_2),a_1,a_2)=U(s_1(X_1),s_2(X_2))-C(a_1,a_2)$, where $U(s_1(X_1),s_2(X_2))$ is the utility of the ISP from the total revenues shared from the CPs and $C(a_1,a_2)$ is the cost incurred for applying the efforts $a_1$ and $a_2$. %As the ISP is generally assumed to be risk averse, then $U(\cdot)$ is strictly concave in both terms.
 
Each $CP$ aims at determining an optimal sharing function (contract) $s_i(.)$ that maximizes its expected net revenue. The optimization problem associated to CP$_i, i=1,2$ is given by the following constraint optimization problem:
\begin{eqnarray} \nonumber
&\max_{a_1,a_2, s_i(\cdot)}E_{X_i}[V_i(X_i-s_i(X_i))]&\\
&\text{ s.t } \hspace{3.5mm} E_{X_1,\;X_2}[H(s_1(X_1),s_2(X_2),a_1,a_2)]\geq \overline{H}&\\ 
&\max_{a_1,a_2}E_{X_1,\;X_2}[H(s_1(X_1),s_2(X_2),a_1,a_2)]. &
\end{eqnarray}
Constraint $(1)$ guarantees to the ISP the minimum expected utility $\overline{H}$ and is called as individual rationality (IR) or the participation constraint. The second constraint is the ISP's  optimization problem and is called as incentive compatibility constraint (IC). It also captures the fact that the CPs cannot observe effort level of the ISP. The structure of the optimization problem is hierarchical and can be studied considering a Stackelberg solution concept. In fact, the principal (here each CP) can be seen as a leader and the agent (here the ISP) as the follower who plays after observing the action of the principal. But in our setting, there is another level of complexity as there are two principals and therefore, it  gives a static game between CPs with shared constraints. Then, the use of generalized Nash Equilibrium Point (GNEP)\cite{GNEP} can be useful in order to analyze the optimal sharing contracts at the principal level considering the agent's action.  It is in general hard to solve this type of complex game for arbitrary sharing function. 

In the following we focus on the linear sharing functions (or contracts). We first consider the case where the ISP differentiates the CPs and puts separate for each of them and then consider the case where the CPs are not differentiated and the ISP puts common efforts for both the CPs. Our former case corresponds to the non-neutral regime and the later to the neutral regime.\\


 

%Let $X_i$ as a random variable with a distribution $F(X_i,a)$, parameterized by the ISP's action with density function $f(X_i,a_i)$ and well defined $f_{a}$ and $f_{aa}$ for all $(X_i,a)$. Also, let $g(X_1,X_2,a)$ be joint density function with well defined $g_{a}$ and $g_{aa}$.
%\\The expected utility of $CP_i$ is given by
%\begin{eqnarray}
%&E_{X_i}[V(X_i-s_i(X_i))]=\int V(X_i-s(X_i))f(X_i,a)dX_i&
%%&=a_i-\int s(X_i)f(X_i,a_i)dX_i&
%\end{eqnarray}
%The expected utility of $ISP$ is given by
%\begin{eqnarray}\nonumber
%&E_{X_1, X_2}[U(\sum_is_i(X_i))-C(a)]&\\
%=\int\int U(\sum_is_i(X_i))g(X_1,X_2,a)dX_1dX_2 - C(a)&
%\end{eqnarray}
%Then we have\\
%For $CP_1$:
%\begin{eqnarray}\nonumber
%&\max_{s_1(X_1)} \hspace{3mm} \int V(X_1-s_1(X_1))f(X_1,a)dX_1&\\\nonumber
%&\text{ s.t } \int \int U(s_1(X_1)+s_2(X_2))g(X_1,X_2,a)dX_1dX_2 - C(a)\geq \overline{H}&\\\nonumber
%&\max_{a}  \int \int U(s_1(X_1)+s_2(X_2))g(X_1,X_2,a)dX_1dX_2 - C(a)&
%\end{eqnarray}
%For $CP_2$:
%\begin{eqnarray}\nonumber
%&\max_{s_2(X_2)}\hspace{3mm}\int V(X_2-s_2(X_2))f(X_2,a_2)dX_2&\\\nonumber
%&\text{ s.t }\int \int U(s_1(X_1)+s_2(X_2))g(X_1,X_2,a)dX_1dX_2 - C(a)\geq \overline{H}&\\\nonumber
%&\max_{a} \int \int U(s_1(X_1)+s_2(X_2))g(X_1,X_2,a)dX_1dX_2 - C(a)&
%\end{eqnarray}
%
%This is a game between $CP_1$ and $CP_2$ having shared constraints. Such a game is called as GNEP.
%Contracts are linear type.

==> Journal Version Arxiv/problem.tex <==
We consider multiple Content Providers (CPs) and a single Internet Service Provider (ISP) that connects end users to the content of the CPs. Each CP can enter into a contract with the ISP under which the ISP agrees to offer a better quality of service on the contents of the CPs to the end users by investing in the network infrastructure \cite{caching} and in turn, each CP agrees to share a part of its revenue with the ISP. One example of ISP investing in network infrastructure to improve QoS is caching, where better caching efforts by the ISP for a CP's content results in higher revenue for the CP. However, such caching decisions (effort or action) of ISP may not be directly visible to the CPs, but each CP can observe the QoS experienced by end users through demand for their contents. Thus, higher the effort (caching) by the ISP, higher will be the revenue for CP because of the price paid for their content or from advertisements (from the click-through rate) \cite{Courcou13}. However, the ISP's profit maximization strategy may not be aligned with the interests of the CPs, and moreover, the ISP effort (that influence CP revenue) is not directly observable by CPs.  This scenario gives rise to the Moral Hazard problem.
%can hide or disguise its effort %and informations are asymmetric. %This may result in inefficient and unstable agreements.

\begin{figure}[h!]
 	\begin{center}
 		\includegraphics[scale=0.4]{figures/figure.png}
 		\caption{Revenue flow between CPs, ISP and End Users.}
	\label{fig:figure1}      
\end{center}
\end{figure}
 
%The ISP connects the end users to the content of the CPs. 
Let $n$ denote the number of CPs and $\mathcal{N}=\{1,2,\dots, n\}$ the set of CPs.  For each $i \in N$ we denote $i$-th CP as $\CPi$. %The ISP must provide the\se two contents to end users. 
%The variable $Q_i$ measures the global average quality of service associated of contents from CP $i$. The ISP can decide to increase $Q_i$ by improving the availability of CP $i$ content through caching efforts for example \cite{caching}. We denote the efforts the ISP puts to improve  the quality $Q_i$ by $a_i$, for each CP $i$ traffic. We assume that higher the efforts higher is the quality perceived by end users accessing content to each CP, i.e., 
%$$ \frac{\partial Q_i}{\partial a_i}>0.$$
%\subsection{CP strategy}
The revenue of $\CPi$ from its content is  random and denoted as $X_i\in \mathcal{R}_+$ with probability density function $F_i$. The amount of efforts put by the ISP to improve the demand for the content of $\CPi$ is quantified by a positive number denoted as $a_i \in \mathcal{R}_+$. %The revenue is assumed to be increasing in $a_i$, i.e., for any realization $x_i$ of $X_i$, $\frac{\partial x_i}{\partial a_i}>0$.
%We denote a realization of $X_i, \; i=1,2$ by $x_i$ and it is assumed that $x_i$ is increasing  content of $\CPi$. Further, we assume that higher the  efforts by the ISP for $\CPi$, the demand for its content will be higher which in turn results in higher revenue $X_i$, i.e.,
% The average revenue generated  expressed in terms of per click revenue as $$X_i=r_iD_iP_i$$
%where, $r_i$ is Revenue per click for $CP_i$, $D_i$ is the averagel demand generated for $CP_i$ and $P_i$ is Probability of click for $CP_i$.\\
%The next schema explains the relationship between the caching strategy $a_i$, the quality of service $QoS_i$ and the revenue $X_i$: 
%$$a_i\Rightarrow QoS_i\Rightarrow X_i.$$
%$$\frac{\partial F_i(x_i | a_i)}{\partial a_i}<0.$$ 
%This assumption implies that the greater effort from the ISP to  $CP_i$s traffic, higher revenue is the  revenue for $CP_i$, i.e. for all $i$, $\frac{\partial x_i}{\partial a_i}>0$. 
$\CPi$ shares part of his revenue with the ISP to incentivize ISP investments. This share is determined by the outcome as sharing function $s_i:\mathcal{R}_+ \rightarrow \mathcal{R}_+$, which is called contract or agreement in the moral hazard framework. Specifically, if $x_i$ is the realized revenue in a month for $\CPi$, it gives  $s_i(x_i)$ to the ISP. Then, the net revenue of $\CPi$ is $x_i-s_i(x_i)$. Our goal in this work is first to design optimal sharing functions $s_i(\cdot), i\in \mathcal{N}$ that maximize the expected net revenues of each CPs taking into account the rational behavior of the ISP and its participation constraints. We assume that the CPs offer a similar type of content and compete with each other to attract more demand.  Our model with multiple CPs and a single ISP is depicted in Figure~\ref{fig:figure1}. In the terminology of moral hazard, the CPs are the principles, and the ISP is the agent. We thus have multiple principles and a single agent.  

\noindent
{\bf Demand and Revenue:} The increment in demand for content of $\CPi$ depends on the effort by the ISP to improve QoS for  $\CPi$ content and could be random. Let $D_i$ denote this increment in demand. We assume that the mean of $D_i$ grows logarithmically in $a_i$ (law of diminishing gains) and is given by $D_i:=\log(a_i+1)+\epsilon_i, i\in \mathcal{N}$,  where $\epsilon_i$ is the random variation in the demand for $\CPi$. 
%We assume that $\epsilon:=(\epsilon_1, \epsilon_2, \ldots, \epsilon_n) $ is jointly Gaussian with mean $0$ and covariance matrix $K$ given by\footnote{$D_i$ can take negative values making demand negative. We ignore this fact as our interest is only in the mean increment in demand. To overcome this operational hurdle, one can use exponential distribution, and similar analysis holds.}
%: \[
%K =
%\left[ {\begin{array}{cc}
%	\sigma_1^2 & \rho \sigma_1\sigma_2 \\
%	\rho \sigma_1\sigma_2 & \sigma_2^2  \\
%	\end{array} } \right].
%\]

The revenue generated for $\CPi$ is proportional to the demand and
given by $X_i=r_iD_i$, where $r_i$ is a constant that captures how
each unit of demand translates to earnings. For example, $r_i$ could
be revenue per click for $\CPi$ when $D_i$ is interpreted as total
number of clicks on $\CPi$'s content. The expected revenue for $\CPi$
is then $\mathbb{E}[X_i]=r_i\log(r_i+1)$.\footnote{Our model
generalizes trivially to the case where $D_i:=
d_i \log(a_i+1)+\epsilon_i,$ i.e., the average demand scales with a
CP-specific multiplicative constant; this constant can simply be
absorbed into $r_i.$}

%Second, the impact of these optimal contracts are studied onto the neutral behavior of the ISP. In fact, optimal contracts may lead to non-neutral behavior of the ISP, in the sense that the ISP will not apply the same action/effort to both traffic. This behavior is typically a non-neutral behavior and is particularly of interest for the net neutrality debate \cite{netneutrality}.  
 

\subsection{Utilities and Objective}
For a given contract $s_i(\cdot), i\in \mathcal{N}$ the net revenue for $CP_i$ is
$X_i-s_i(X_i)$. Let $V_i(\cdot)\in\mathcal{R}$ denote the utility
function of $\CPi$ and is typically assumed to an increasing concave
function of the $CP$'s net revenue. We assume the utility of $CP_i$ is
linear in its net revenue and set
$V_i(X_i-s_i(X_i))=X_i-s_i(X_i)$. The utility of the ISP depends on
revenue-share it receives from both the CPs and also the cost involved
in the efforts it puts for the CPs. The earning for the ISP from the
CPs is $\sum_{i} s_i(X_i)$ while it incurs a total cost of
$c\sum_{i}a_i$, where $c$ is a positive constant. The net earnings for the ISP
is then $W(s_1(X_1) \ldots,s_n(X_n),a_1\ldots, a_n)=\sum_{i}
s_i(X_i)-c\sum_{i}a_i$. We assume the ISP is risk-averse and set its
utility as $H(W)=-\exp\{-zW\}$, where $z$ is a risk-averse
parameter. This utility is referred to as Constant Absolute Risk
Aversion (CARA) in the literature \cite{rabin2013risk}. The ISP enters
into agreement with the CPs only if its expected utility is larger
than a certain threshold denoted as $\overline{H}$.

The CPs compete against each other and aim to maximize their utility. The objective of $\CPi, i\in \mathcal{N}$ taking into participation constraints of the ISP is given as follows:
\begin{eqnarray} \nonumber
&\max_{a_1,...,a_n, s_i(\cdot)}\UCPi:=\mathbb{E}_{X_i}[V_i(X_i-s_i(X_i))]&\\
&\hspace{-5mm}\text{subjected to} \hspace{1mm} \mathbb{E}_{X_1,...,X_n}[H(s_1(X_1),...,s_n(X_n),a_1,...,a_n)]\geq \overline{H}& \label{eqn:IR}\\ 
&\max_{a_1,\ldots,a_2}\mathbb{E}_{X_1,...,X_n}[H(s_1(X_1),...,s_n(X_n),a_1,...,a_n)]. &  \label{eqn:IC}
\end{eqnarray}
Constraint (\ref{eqn:IR}) guarantees the ISP minimum expected utility $\overline{H}$ and is called as individual rationality (IR) or the participation constraint. The second constraint (\ref{eqn:IC}) is the ISP's optimization problem and is called an incentive compatibility constraint (IC). It also captures the fact that the CPs cannot observe the effort level of the ISP. Note that the Constraint in (\ref{eqn:IC}) may have multiple optima hence objective of each CP is optimized over all of these possibilities.  The structure of the optimization problem is hierarchical and can be studied considering a Stackelberg solution concept where the principals (here each CP) can be seen as leaders and the agent (here the ISP) as the follower who plays after observing the action of the principals. In our setting, there is another level of complexity as there are multiple strategic principals. This gives rise to a static game between CPs with shared constraints.

%Then, the use of generalized Nash Equilibrium Point (GNEP)\cite{GNEP} can be useful in order to analyze the optimal sharing contracts at the principal level considering the agent's action.  It is in general hard to solve this type of complex game for arbitrary sharing function. 

%In the following we focus on the linear sharing functions (or contracts). We first consider the case where the ISP differentiates the CPs and puts separate for each of them and then consider the case where the CPs are not differentiated and the ISP puts common efforts for both the CPs. Our former case corresponds to the non-neutral regime and the later to the neutral regime.\\




\subsection{Linear Contracts}
In the following we consider a specific type of contract where CPs
share a fraction of their revenue to ISP. These contracts are of the form
$s_i(X_i)=\beta_i X_i$ and are referred to as linear contracts, where
$\beta_i\in [0,1]$ for all $i\in \mathcal{N}$. The ISP chooses whether to accept
or reject the contract. Linear contracts are shown to be optimal
in \cite{holmstrom1991multitask} particularly when agent has a risk
averse utility which is also the case in our setting. Henceforth we denote a linear contract between the ISP and $\CPi$ by its parameter
$\beta_i$.  The expected utility of $CP_i$ is then:
\begin{align*}
\UCPi =\mathbb{E}[X_i(1-\beta_i)]=(1-\beta_i)r_i\log(a_i+1),
\end{align*}
%\begin{eqnarray}\nonumber 
%&E[V(X_i-s_i(X_i))]=E[V(X_i-(\alpha_i+\beta_i X_i))]&\\
%& =E[X_i(1-\beta_i)-\alpha_i] =(1-\beta_i)r_i\log(a_i+1)-\alpha
%_i,&
%\end{eqnarray}
and the expected utility of the $ISP$ is:
\begin{align*}
&\UISP=\mathbb{E}\left [H\left(\sum_{i} (s_i(X_i)-ca_i)\right)\right] \\
&=E\left [H\left (\sum_i(\beta_ir_i(\log(a_i+1)+\epsilon_i)-ca_i)\right)\right]\\
%&=E\left[-\exp\left(\sum_i(\beta_ir_i(\log(a_i+1)+\epsilon_i)-ca_i)\right)\right ]\\
&=-\exp\left\{-z\sum_i(\beta_ir_i\log(a_i+1)-ca_i)\right\} \mathbb{E}\left[\exp\left\{-z\sum_i\beta_ir_i\epsilon_i\right\}\right].
\end{align*}
%The expression for the expected utility for the ISP follows after noting that last part of it is the characteristic function of a Gaussian random vector. 
The ISP's optimization problem is to find an effort level $a_i$ for each CP$_i$ which maximizes its expected
utility. Notice that maximizing expected utility (IC constraint) is
equivalent to maximizing $\sum_i(\beta_ir_i\log(a_i+1)-ca_i)$ over
$(a_1,\ldots, a_n)$.
%$$
%\sum_i[\beta_ir_i\log(a_i+1)-ca_i]-\frac{z}{2}[(\beta_1r_1\sigma_1)^2+(\beta_2r_2\sigma_2)^2+2\rho\beta_1\beta_2r_1r_2\sigma_1\sigma_2]
%$$\\
%\noindent

\subsection{Neutral vs Non-Neutral regime}
We distinguish two scenarios based on differentiation in the efforts by the ISP for each CP. We say that the network is {\em neutral} if ISP puts the same amount of efforts for both the CPs irrespective of the revenue-share it can get from them, i.e., ISP always sets $a_1=a_2...=a_n$. We say that the network is {\em non-neutral} if the ISP can put different amount of effort for each CP, i.e., $a_1\neq a_2...\ne a_n$ is permitted. Hence in the neutral regime the ISP treats each CP identically, whereas it can differentiate between them in the non-neutral regime. 

Under the neutral regime and linear contracts, the IC constraint of the ISP, i.e., $\max_{a}E[H(s_1(X_1),...,s_n(X_n),a)]$, simplifies  to $\max_a \sum_i(\beta_ir_i\log(a+1)-ca)$. The optimal effort level for a given contracts $(\beta_i, i\in \mathcal{N})$ is given by:
	\begin{equation}
a^*=\max\left(\frac{\sum_i\beta_ir_i}{nc}-1,0\right).
\end{equation}
The objective function of $\CPi, i\in \mathcal{N}
$ in the neutral regime can then be expressed as follows:\\
\vspace{.2cm}
\textbf{Neutral:}
\vspace{-.2cm}
\begin{equation}
\label{eqn:OptNeutral}
\begin{aligned}
 &\max_{\beta_i \in [0,1]} \hspace{2mm} (1-\beta_i)\log(a+1)r_i\\
&\text{subjected to} \sum_iz(\beta_ir_i\log(a+1)-ca)\\
&-\log\mathbb{E}\left[\exp\left\{-z\sum_i\beta_ir_i\epsilon_i\right\}\right]\geq -\log (-\overline{H})\\
& \text{ and } a=\max\left(\frac{\sum_i\beta_ir_i}{nc}-1,0\right).\\
%&\hspace{10mm}-\frac{z}{2}[(\beta_1r_1\sigma_1)^2+(\beta_2r_2\sigma_2)^2+2\rho\beta_1\beta_2r_1r_2\sigma_1\sigma_2]\\
%&\hspace{20mm}\text{where} %\hspace{1.5mm}\overline{h}=-\log (-\overline{H}).
\end{aligned} 
\end{equation}
Under the non-neutral regime, the IC constraint of the ISP, i.e., $\max_{a_1,\ldots, a_n}E[H(s_1(X_1),...,s_n(X_n),a_1,...,a_n)]$, simplifies  to $\max_{a_1,\ldots,a_n} \sum_i(\beta_ir_i\log(a_i+1)-ca_i)$.  The optimial efforts level for a given contracts $(\beta_i, i\in \mathcal{N})$ are:
$$a_i^*=\max\left(\frac{\beta_ir_i}{c}-1,0\right) \mbox{ for }  i\in \mathcal{N}.$$
Simplified optimization problem for  each $CP_i$ can then be expressed as the following bi-level optimization problem: \\
\vspace{.2cm}
\textbf{NonNeutral:}
\vspace{-.2cm}
\begin{equation}
\label{eqn:OptNonNeutral}
\begin{aligned}
&\max_{\beta_i \in [0,1]} \hspace{2mm} (1-\beta_i)\log(a_i+1)r_i\\
&\text{subjected to} \sum_i z(\beta_ir_i\log(a_i+1)-ca_i)\\
&-\log\mathbb{E}\left[\exp\left\{-z\sum_i\beta_ir_i\epsilon_i\right\}\right]\geq -\log (-\overline{H})\\
&\text{ and } a_i=\max\left(\frac{\beta_ir_i}{c}-1,0\right) \mbox{ for } i \in \mathcal{N}.
%&\hspace{10mm}-\frac{z}{2}[(\beta_1r_1\sigma_1)^2+(\beta_2r_2\sigma_2)^2+2\rho\beta_1\beta_2r_1r_2\sigma_1\sigma_2]\\
%&\hspace{20mm}\text{where} %\hspace{1.5mm}\overline{h}=-\log (-\overline{H}).
\end{aligned}
\end{equation} 
Notice that the ISP has incentive to enter into contract with the CPs only when $\overline{H}\geq -1$, otherwise its net earning from the CPs is negative
For any value of $\overline{H} \in (-1, 0]$, the IR constraint make the strategies of the players coupled and the game can have continuum of equilibria as it is the case with general coupled constrained games \cite{GNEP}. However, with continuum of equilibria we will be faced with equilibrium selection problem and a systematic comparison of CP utilities under the two regime is not possible. We thus set $\overline{H}=-1$ under which the IC constraint ensures that the IR constraint always holds and hence the objective of the CPs are no more jointly constrained. As we will see in the subsequent sections, this avoids the continuum of equilibrium. We note that even after relaxing the IR constraint the problem is still challenging to analyze,  but makes it possible to compare equilibrium utilities of all players under both the regimes. 

%In the following we assume that $\overline{H}=-1$ so that the IR constraint is active whenever net earning for the ISP is non-negative. This removes the possibility of  continuum of equilibrium that arises in the games with such coupled constraints \cite{GNEP}. With existence of continuum of equilibrium we will be faced with the equilibrium selection problem and a systematic comparison of utilities is not possible. 

We say that a contract profile $(\beta_i,i\in \mathcal{N})$ is an equilibrium if no CP has an incentive for unilateral deviation from its contract. In the following we superscript the quantities computed at equilibrium with NN and N when they are associated with non-neutral regime and neutral regime respectively. 
 

% is met whenever  \textcolor{red}{Then, it is natural to consider that $\overline{H}=-1$ and the IR constraint becomes a positivity constraint.} \textbf{Why this is natural?}

%For any value of $\overline{H} \in (-1, 0]$, the IR constraint make the strategies of the both the players coupled and the game can have continuum of equilibria as it is the case with general coupled constrained games \cite{GNEP}. However, with continuum of equilibria the comparison of CP utilities under the two regime is not possible. We thus set $\overline{H}=-1$ under which the IC constraint ensures that the IR constraint always holds and hence the objective of the two CPs are no more jointly constrained. As we will see in the subsequent sections, this avoids the continuum of equilibrium and allows a comparison of the utilities of the players in different regimes. 
 
%An important assumption is that the ISP will accept the CP$_i$ contract if and only if his expected net utility $E(s_i(X_i)-ca_i)$ obtained from CP$_i$ is positive. Hence, if $\sum_i[s_i(X_i)-ca_i]) \geq 0$, the ISP will accept both contracts. Considering this natural case (other case is not of interest here as there is only one CP and then no game between several CPs), yields that for all risk averse parameter $z$, the ISP utility $H(W)\geq -1$ and a natural minimum expected utility is $\overline{H}:=-1$. 


==> Journal Version Arxiv/symmetric.tex <==
In this section, we consider the special case where CPs are symmetric in terms of their monetization power , i.e., $(r_1=r_2=r)$ and compare the utilities of CPs and ISP in non-neutral and neutral regimes. The following corollary to Thm.~\ref{Thm:NN-asy} gives the equilibrium contracts in the non-neutral regime.
%\subsection{Non-Neutral regime}
%In this section, we consider that ISP is allowed to make different investment $a_i$ for each CP$_i ; i=1,2$. The problem for each $CP_i$ reduces to 
%\begin{align*}
%&\hspace{8.9mm}\max_{a_1, a_2 \beta_i} \hspace{3mm} (1-\beta_i)r\log(a_i+1)\\
%&\text{s.t.}\\
%&\text{argmax}_{a_1,a_2}\hspace{3mm} \sum_iz\left(\beta_ir\log(a_i+1)-ca_i\right)
%\end{align*}
%%\begin{eqnarray}
%%\nonumber&\max_{a_i, \beta_i} \hspace{2mm} (1-\beta_i)\log(a+1)r&\\\nonumber \noindent
%%&\max_{a_1,a_2}\hspace{3mm} \sum_iz\left(\beta_ir\log(a_i+1)-ca_i\right)&\\
%%\end{eqnarray}
%Following Lemma gives the equilibrium solution 
\begin{corollary} \label{lma:NN-sym}
	In the non-neutral regime equilibrium contract is given by 
	\begin{equation}
	\beta_1^{NN}=\beta_2^{NN}=\begin{cases}
	0  &\mbox{  if }  \frac{r}{c}\leq 1, \\
	\frac{1}{W\left(\frac{r}{c}e\right)}  &\mbox{  if }  \frac{r}{c} > 1,
	\end{cases}
	\end{equation}
	where $W(\cdot)$ is the Lambertw function. Further, the effort levels of the ISP for are given by
	\begin{equation} \label{eqn:NN-a}
a_i^{NN}=a^{NN}=\max\left(\frac{\beta^{NN} r}{c}-1,0\right) \hspace{1.5mm} \forall i=1,2.
\end{equation}
\end{corollary}
%\begin{lemma} \label{lma:NN-sym}
%	The investment decision	of ISP for each CP$_i; i=1,2$ is given by
%	\begin{equation} \label{eqn:NN-a}
%	a_i^{NN}=a^{NN}=\max\left(\frac{\beta^{NN} r}{c}-1,0\right) \hspace{1.5mm} \forall i=1,2
%	\end{equation}
%	and the share proportion for both CPs are equal and is given by:	
%\begin{equation}
%\beta_i^{NN}=\beta^{NN}=\begin{cases}
%0  &\mbox{  if }  \frac{r}{c}\leq 1, \\
%\frac{1}{W\left(\frac{r}{c}e\right)}  &\mbox{  if }  \frac{r}{c} > 1
%\end{cases}
%\end{equation}
%where $W(\cdot)$ is the Lambertw function.
%%	\begin{equation}
%%	\beta_i^{NN}=\beta^{NN}=\frac{1}{W\left(\frac{r}{c}e\right)} \hspace{2mm} \forall \hspace{1mm}  \frac{r}{c}>1
%%	\end{equation}
%%		\begin{equation}
%%	\beta_i^{NN}=\beta^{NN}=0\hspace{2mm} \forall \hspace{1mm}  \frac{r}{c}\le 1
%%	\end{equation}
%\end{lemma}

Now, utility of each $\CPi,i=1,2$ at equilibrium is given by
\begin{eqnarray}\nonumber
\UCPi=(1-\beta^{NN}) r\log(a^{NN}+1)=\frac{(1-\beta^{NN})^2}{\beta^{NN}}r,
\end{eqnarray}
and utility of the ISP at equilibrium is give by:
\begin{eqnarray}\nonumber
&\UISP=\left[2\beta^{NN} r \
\log(a^{NN}+1)-c(2a^{NN})\right]&\\
&=\left[2(r+c)-4\beta^{NN}r\right].
\end{eqnarray}

%%
%\subsection{Neutral regime}
%In this section, we consider that ISP is allowed to make different investment $a_i$ for each CP$_i ; i=1,2$. The problem for each $CP_i$ reduces to 
%\begin{align*}
%&\hspace{8mm}\max_{a, \beta_i} \hspace{2mm} (1-\beta_i)\log(a+1)r\\
%&\text{s.t.}\\
%&\text{argmax}_{a}\hspace{3mm} z\left(\sum_i\beta_ir\log(a+1)-2ca\right)
%\end{align*}
%
%%\begin{eqnarray}
%%\nonumber&\max_{a, \beta_i} \hspace{2mm} (1-\beta_i)\log(a+1)r&\\\nonumber \noindent
%%&\text{s.t.}&\\\nonumber
%%&\text{argmax}_{a}\hspace{3mm} \sum_iz\left(\beta_ir\log(a+1)-2ca\right)&\\
%%\end{eqnarray}
The following corollary to Thm.~\ref{Thm:Neutral-asym} specializes the results in the neutral regime.
\begin{lemma} \label{lma:N-sym}
	The equlibrium contracts in the neutral regime is given by:	
\begin{equation}
\beta_i^{N}=\beta^{N}=\begin{cases}
0  &\mbox{  if }  \frac{r}{2c}\leq 1, \\
\frac{1}{2W\left(\frac{r}{2c}e^{0.5}\right)}  &\mbox{  if }  \frac{r}{2c} > 1
\end{cases}
\end{equation}
and the common effort level by the ISP is given by
\begin{equation} \label{eqn:N-a}
a^{N}=\frac{\beta^{N} r}{c}-1
\end{equation} 
%	\begin{equation}
%	\beta^{N}=\frac{1}{2W\left(\frac{r}{2c}e^{0.5}\right)}
%	\end{equation}
\end{lemma}
Utility of each CP at equilibrium is then 
\begin{eqnarray}\nonumber
(1-\beta^{N}) r\log(a^{N}+1)
=\frac{(1-\beta^{N})^2}{2\beta^{N}}r
\end{eqnarray}
and the ISP utility is:
\begin{eqnarray}\nonumber
\left[2\beta^{N} r \log(a^{N}+1)-2c(a^{N})\right]=\left[r+2c-3\beta^{N}r\right].
\end{eqnarray}  \subsection{Comparison between Non-neutral and neutral regime}
In this section we study the comparison between Non-neutral and neutral regime when CPs are symmetric and have same revenue per click rates.

%\begin{figure*}[!tb]
%	\centering
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig1}%
%		\label{fig:effort}}
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig2}%
%		\label{fig:beta}}
%		\hspace{0.55cm}
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig3}%
%		\label{fig:beta}}
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig4}%
%		\label{fig:Utility1}}
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig5}%
%		\label{fig:Utility2}}
%	%		\subfloat[]{\includegraphics[scale=0.04]{figures/Gain3}%
%	%		\label{fig:Gain4}}
%	\caption {Comparison between Non-neutral and neutral w.r.t c}
%	\label{fig:Gain}
%\end{figure*}
%
%\begin{figure*}[!tb]
%	\centering
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig2a}%
%		\label{fig:effort}}
%		\subfloat[]{\includegraphics[scale=0.4]{figures/Fig2e}%
%		\label{fig:beta}}
%	\hspace{0.55cm}
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig2b}%
%		\label{fig:Utility1}}
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig2c}%
%		\label{fig:Utility2}}
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig2d}%
%		\label{fig:Utility2}}
%	
%	\caption {Comparison between Non-neutral and neutral w.r.t $r$}
%	\label{fig:Gain}
%\end{figure*} 

\begin{lemma} \label{lma:betacomp}
Proportion of revenue shared by each CP in higher in non-neutral regime as compared to that in neutral regime, i.e.,	$$\beta^{NN} \geq {\beta^{N}}$$
\end{lemma}
Above lemma suggest that CPs share more revenue in non-neutral regime as compared to neutral regime.

\begin{lemma} \label{lma:effortcomp}
	ISP makes more investment in higher in non-neutral regime as compared to that in neutral regime, i.e.,	$$a^{NN} \geq {a^{N}}$$
\end{lemma} 

Proof of above lemma follows directly. Since, investment decision by ISP is monotonically increasing in shared revenue proportion (from eqns. (\ref{eqn:NN-a}) and (\ref{eqn:N-a})), by lemma \ref{lma:betacomp} it is clear that ISP  make more investment in non-neutral regime as compared to neutral regime.

\begin{lemma} \label{lma:UISPcomp}
	Utility of ISP is higher in non-neutral regime as compared to that in neutral regime.
\end{lemma}

\begin{lemma} \label{lma:UCPcomp}
	Utility of each CP is higher in non-neutral regime as compared to that in neutral regime.
\end{lemma}

==> bargaining.tex <==
In this section, we consider the cooperative scenario where CPs in the neutral regime bargain to arrive at an agreement on their revenue share proportions to be given to ISP. We use the classical cooperative solution concept, the Nash Bargaining solution \cite{NBS}.
A Nash Bargaining solution $(\beta_1^B,\beta_2^B)$ is defined as the solution of the following maximization problem:
\begin{align*}
\max_{\beta_1,\beta_2} &\hspace{2mm} (U_{CP_1}-d_{CP_1})(U_{CP_2}-d_{CP_2})\\
&\text{s.t.}\hspace{4mm}(U_{CP_1},U_{CP_1})\in \mathcal{S}\\
&\hspace{4mm} 0 \le\beta_1\le 1,0 \le \beta_2 \le 1
\end{align*}
where $\mathcal{S}$ of the set of all feasible, non-negative utility vectors given by $$\mathcal{S}:=\{(U_{CP_1}(\beta_1,\beta_2),U_{CP_2}(\beta_1,\beta_2))| \hspace{0.5mm}0\leq \beta_1\leq1,0\leq\beta_2\leq 1\} \cap \mathbb{R}^2_+$$
and $d_{CP_i} ; i=1,2$ are disagreement points. In our case, the disagreement points correspond to the utility that the CP$_i$ gets when fails to arrive at an agreement to share revenue proportion with ISP. These are equal to zero ($d_{CP_1}=d_{CP_2}=0$), since when no revenue is shared by CPs, there is no investment (effort) by ISP in the network and utility of each CP is zero.
\subsection{Symmetric case}
In this section, we consider the Nash Bargaining Problem (NBP) between the CPs when they are symmetric with respect to revenue per click rates, i.e., $r_1=r_2=r$. For this case, given ISP investment decision, NBP between CPs is given as follows:
\begin{align*}
\max_{\beta_1,\beta_2} &\hspace{2mm} (1-\beta_1)(1-\beta_2)r^2\left[\log\left(\frac{(\beta_1+\beta_2)r}{2c}\right)\right]^2\\
&\text{s.t.}\hspace{10mm} 0 \le\beta_1\le 1,0 \le \beta_2 \le 1
\end{align*}

\begin{thm} \label{thm:NBS1}
	The NBS of the above NBP is given as:
	$$\beta_1^B=\beta_2^B=\beta^B=\frac{1}{W\left(\frac{r}{c}e\right)}  \hspace{1mm} \forall \frac{r}{c}>1
$$

\end{thm}

%%
\subsection{General case}
In this section, we consider the Nash Bargaining Problem (NBP) between the CPs when they are asymmetric with respect to revenue per click rates, i.e., $r_1\ne r_2$, and without loss of generality we assume that $r_1>r_2$. For this case, given ISP investment decision, NBP between CPs is given as follows:
\begin{align*}
\max_{\beta_1,\beta_2} &\hspace{2mm} (1-\beta_1)(1-\beta_2)r_1r_2\left[\log\left(\frac{\beta_1r_1+\beta_2r_2}{2c}\right)\right]^2\\
&\text{s.t.}\hspace{13mm} 0 \le\beta_1\le 1,0 \le \beta_2 \le 1
\end{align*}

\begin{thm} \label{thm:NBS2}
	The NBS of the above NBP is given as:
	\begin{equation}
(\beta_1^B,\beta_2^B)=\begin{cases}
\overline{\beta}_1^B, \overline{\beta}_2^B &\mbox{  if }  \frac{r_1+r_2}{r_1-r_2} > W\left(\frac{r_1+r_2}{2c}e\right), \\
(\hat{\beta}_1^B,0)  &\mbox{  else }  
\end{cases}
\end{equation}
where
\begin{equation}\nonumber
\overline{\beta}_1^B=\frac{r_1+r_2}{2r_1W\left(\frac{r_1+r_2}{2c}e\right)}-\frac{r_2-r_1}{2r_1}
\end{equation}
\begin{equation} \nonumber
\overline{\beta}_2^B=\frac{r_1+r_2}{2r_2
	W\left(\frac{r_1+r_2}{2c}e\right)}-\frac{r_1-r_2}{2r_2}
\end{equation}
$$
\hat{\beta}_1^B=\frac{2}{
	W\left(\frac{r_1}{c}e^2\right)}
$$
\end{thm}

It is not necessary that disagreement point is $(0,0)$, it is possible when CPs don't agree on the bargaining contract, they may act non-cooperatively and in that case disagreement point is the equilibrium solution of the non-cooperative game between CPs. 
fo
\begin{figure*}[h!] 
	\centering
	{\includegraphics[scale=0.35]{figures/b1}%
	}
	{\includegraphics[scale=0.35]{figures/b2}%
}
	{\includegraphics[scale=0.35]{figures/A}%
}
	{\includegraphics[scale=0.35]{figures/CP1U}%
}
{\includegraphics[scale=0.35]{figures/CP2U}%
}
{\includegraphics[scale=0.35]{figures/ISP}%
}
{\includegraphics[scale=0.35]{figures/ScU}%
}
	\caption {Comparison between Non-neutral, neutral and bargaining setup when CPs are asymmetric when disagreement point is $(0,0)$. We fix $c=1, r_2=2$ and vary $r_1$ from 2 to 30.}
%	\label{fig:comparisonISP}
\end{figure*}

\begin{figure*}[h!] 
	\centering
	{\includegraphics[scale=0.35]{figures/beta1nbs}%
	}
	{\includegraphics[scale=0.35]{figures/beta2nbs}%
	}
	{\includegraphics[scale=0.35]{figures/totaleffortb}%
	}
	{\includegraphics[scale=0.35]{figures/CP1Ub}%
	}
	{\includegraphics[scale=0.35]{figures/CP2Ub}%
	}
	{\includegraphics[scale=0.35]{figures/ISPUb}%
	}
	{\includegraphics[scale=0.35]{figures/SUb}%
	}
	\caption {Comparison between Non-neutral, neutral and bargaining setup when CPs are asymmetric and disagreement point is Nash Equilibrium. We fix $c=1, r_2=2$ and vary $r_1$ from 2 to 10.}
\end{figure*}



%\begin{figure*}[h!] 
%	\centering
%	{\includegraphics[scale=0.35]{figures/CP1U}%
%	}
%	{\includegraphics[scale=0.35]{figures/CP2U}%
%	}
%	{\includegraphics[scale=0.35]{figures/ISP}%
%	}
%	{\includegraphics[scale=0.35]{figures/ScU}%
%}
%	\caption {Comparison between Non-neutral, neutral and bargaining setup when CPs are asymmetric. We fix $c=1, r_2=2$ and vary $r_1$ from 2 to 20.}
%	%	\label{fig:comparisonISP}
%\end{figure*}

==> forcing_neutrality.tex <==

Competition between CPs induces non-neutral behavior in separate effort case, i.e. different effort made by the ISP for each CP ($a_1 \neq a_2$). In this case, neutrality can be imposed by making the same effort of the ISP for both CPs equal. We can think about an external control done by an entity (the governmental authority for example). This external entity may impose a tax on the contents such that the resulting investment strategy of the ISP is neutral, i.e. $a^*_1=a^*_2$. We can then think about a three layers hierarchical game where:
\begin{enumerate}
	\item At the higher level (authority level), the authority determines the taxes that each CP$_i$ has to pay on their benefit (for example a percentage of the net profit, say $t_i$) in order to minimize the difference between $a_1^*$ and $a_2^*$.
	\item At the intermediate level, based on this tax, each CP $i$ determines the optimal contract $s_i(.)$ with the ISP.
	\item Finally, at the lower level, the ISP determines optimally his investment $a_i$ for each CP$_i$ traffic.
\end{enumerate}
The problem for CP$_i$ is give as
\begin{align*}
&\hspace{10mm}\max_{a_1, a_2 \beta_i} \hspace{2mm} (1-\beta_i)(1-t_i)r_i\log(a+1)\\
&\text{s.t.}\\
&\text{argmax}_{a_1,a_2}\hspace{3mm} \sum_iz\left(\beta_i(1-t_i)r_i\log(a_i+1)-ca_i\right)
\end{align*}
\begin{lemma}
	The action by ISP for each $CP_i$ is given by\\ 
	%$$
	%\beta_1^*=\frac{c(a_1^*+a_2^*)}{r_1P_1}, \beta_2=\frac{c(a_1^*+a_2^*)}{r_2P_2}
	%$$
	\begin{equation}
	a_i+1=\max\left(\frac{\beta_ir_i(1-t_i)}{c},1\right) , i=1,2
	\end{equation}
\end{lemma}
\begin{lemma}
	The equilibrium solution of the above problem is given as:
	\begin{equation}
		(\beta_1^*,\beta_2^*)=\begin{cases}
		0  &\mbox{  if }  \frac{r_i(1-t_i)}{c}\leq 1 \forall i=1,2, \\
		\left(\frac{1}{W\left(\frac{r_1(1-t_1)}{c}e\right)}, 0\right)  &\mbox{  if }  \frac{r_1(1-t_1)}{c} > 1, \frac{r_2(1-t_2)}{c} \le 1 
		\\
		\left(0, \frac{1}{W\left(\frac{r_2(1-t_2)}{c}e\right)}\right)  &\mbox{  if }  \frac{r_1(1-t_1)}{c} \le 1, \frac{r_2(1-t_2)}{c} > 1 
		\\
		\left(\frac{1}{W\left(\frac{r_1(1-t_1)}{c}e\right)}, \frac{1}{W\left(\frac{r_2(1-t_2)}{c}e\right)}\right)  &\mbox{  if }  \frac{r_1(1-t_1)}{c}>1,  \frac{r_2(1-t_2)}{c}>1 
	\end{cases}
	\end{equation}
\end{lemma}
\begin{lemma}
	The tax $t_i$ for each CP$_i; i=1,2$ is imposed s.t.
	$$e^{W\left(\frac{r_2(1-t_2)}{c}e\right)-W\left(\frac{r_1(1-t_1)}{c}e\right)}=\frac{r_2}{r_1}   $$
\end{lemma}

==> general.tex <==

In this subsection we compare the contracts, utilities of the CPs and the
ISP, and the social utility at equilibrium obtained under the neutral
and the non-neutral regime. We focus on the case of $n=2$ for comparing the non-neutral and neutral regime. Without loss of generality, we assume $r_1 \geq r_2$, i.e.,
$\mbox{CP}_1$ earns higher per unit demand than $\mbox{CP}_2$. We
refer to $\mbox{CP}_1$ as the dominant CP and $\mbox{CP}_2$ as the
non-dominant CP. \textcolor{red}{This constraint will be considered for the rest of
the paper.} What does this line mean?
%We begin with the non-neutral regime. 

%\subsection{Non-neutral regime}
%Under the non-neutral regime, it is easy to see that when
%$\overline{H}=-1$, the CP decisions are no more coupled. The
%optimization problem for $CP_i, i=1,2$ simplifies to:
%\begin{align*}
%&\max_{\beta_i\in [0,1]} \hspace{2mm} (1-\beta_i)r_i\log\left(\max\left(\frac{\beta_ir_i}{c}-1,0\right)+1\right).
%\end{align*}
%Let  $W(\cdot)$ denote the stand LambertW function \textcolor{blue}{\cite{}} taking values on the principle branch. The optimal contract is characterized in term LambertW function in the following. %Each CP has his own constraint optimization problem with common constraint which is the optimization problem of the ISP. Then, the global problem can be seen as a hierarchical non-cooperative game between CPs (here 2 leaders) and one ISP (one follower).Usually, this type of complex game involves the framework of Generalized Nash Equilibrium Point (GNEP) and tools from it mainly for optimization theory and KKT conditions. In our setting, we are able to determine explicitly the equilibrium solution of this hierarchical game between two CPs and one ISP.

\begin{cor}
\label{cor:NN-asy}
In the non-neutral regime, $\CPi, i=1, 2,$ shares a positive fraction
of the revenue at equilibrium with the ISP if and only if $r_i/c
>1$. Specifically, the equilibrium contract is as follows (recall that
$r_1 \geq r_2)$:
	\begin{equation}
(\beta_1^*,\beta_2^*)=\begin{cases}
(0,0)  &\mbox{  if }  \frac{r_i}{c}\leq 1 \forall i=1,2, \\
\left(\frac{1}{W\left(\frac{r_1}{c}e\right)}, 0\right)  &\mbox{  if }  \frac{r_1}{c} > 1, \frac{r_2}{c} \le 1, 
%\\
%\left(0, \frac{1}{W\left(\frac{r_2}{c}e\right)}\right)  &\mbox{  if }  \frac{r_%1}{c} \le 1, \frac{r_2}{c} > 1, 
\\
\left(\frac{1}{W\left(\frac{r_1}{c}e\right)}, \frac{1}{W\left(\frac{r_2}{c}e\right)}\right)  &\mbox{  if }  \frac{r_1}{c}>1,  \frac{r_2}{c}>1,
\end{cases}
\end{equation}	
where $W(\cdot)$ denotes the standard LambertW function \cite{corless1996lambertw}.
\end{cor}
\noindent
Notice that if $r_i$ increases, $\beta_i^*$ decreases, i.e., $\CPi$
shares a small fraction of its revenue with the ISP.
\textcolor{red}{This is because if a CP's capability to translate its demand to
earning improves, then it may require less effort from the ISP to
improve demand for its content and hence can reduce the incentives it
gives through revenue-sharing.}
\textbf{JK: Not obvious here that decreasing $\beta$ implies decreasing
effort! (see the first equation on this column)}


%\subsection{Neutral Regime}
%In the neutral regime, ISP is forced to make the same investment
%decision for both CPs, i.e., $a_1=a_2=a$. The optimization problem for
%CP $i$ in this case simplifies to:
%\begin{align*}
%&\max_{\beta_i \in [0,1]} \hspace{2mm} (1-\beta_i)\log\left(\max\left(\frac{\beta_1r_1+\beta_2r_2}{2c}-1,0\right)+1\right)r_i.
%\end{align*} 
The following theorem gives  equilibrium contracts at equilibrium in the neutral regime for two CPs..

\begin{thm} \label{Thm:Neutral-asym}
Let $r_1 \geq r_2$ and $\frac{r_i}{c} > 1$ for all $i$. If
	$\frac{r_1}{2c}>1,$ then the equilibrium contract in the
	neutral regime is given by:\\ \begin{equation}
	(\beta_1^*,\beta_2^*)=\begin{cases}
	(\overline{\beta}_1, \overline{\beta}_2) &\mbox{ if
	} \frac{r_1+r_2}{r_1-r_2} >
	2W\left(\frac{r_1+r_2}{4c}\sqrt{e}\right), \\ \left(\frac{1}{
	W\left(\frac{r_1}{2c}e\right)},0\right) &\mbox{
	otherwise}, \end{cases} \label{eqn:NeutralConds} \end{equation}
	where \begin{equation}\nonumber \overline{\beta}_1=\frac{r_1+r_2}{4r_1W\left(\frac{r_1+r_2}{4c}\sqrt{e}\right)}-\frac{r_2-r_1}{2r_1}, \overline{\beta}_2=\frac{r_1+r_2}{4r_2
	W\left(\frac{r_1+r_2}{4c}\sqrt{e}\right)}-\frac{r_1-r_2}{2r_2}.  \end{equation}
	Otherwise, the equilibrium contract is
	$(\beta_1^*,\beta_2^*)=(0,0)$, i.e., none of the CPs will
	share their revenue with the ISP.
\end{thm}
In the following we use the notation $(\beta_1^N, \beta_2^N)$ and $(\beta_1^{NN}, \beta_2^{NN})$ to denote the equilibrium contract profiles in the neutral and non-neutral regimes, respectively. Further, we superscript all quantities evaluated under the neutral regime by $N$ and those computed under non-neutral regime by $NN$. For notational convenience let $r_1^*:=r_1^*(r_2)$ denote the value of $r_1$ that satisfies the following relation for a given $r_2$
$$\frac{r_1+r_2}{r_1-r_2} = 2W\left(\frac{r_1+r_2}{4c}\sqrt{e}\right).$$
For $r_1\leq r_1^*$ the first condition in (\ref{eqn:NeutralConds}) is satisfied where revenue shared by  both the CPs is strictly positive, i.e., $\beta_i^{N}>0$ for all $i=1,2$. For $r_1 > r_1^*$ the second condition holds in which only the $\mbox{CP}_1$'s share is strictly positive and $\mbox{CP}_2$ does not share anything, i.e., $\beta_1^N>0$ and $\beta_2^N=0$. Further, it is easy to verify that $r_1^*$ is monotonically increasing in $r_2$ and $r_1^*>  r_2$.
%The above theorem gives equilibrium of the game between CPs under the assumption that $\frac{r_i}{c} > 1 \forall i=1,2$, $\frac{r_i}{2c}>1$ for at least one $i$. 


==> linear.tex <==
In this section, we consider special case that $CP_i$ offers a linear contract to ISP of the form $s_i(X_i)=\beta_i X_i$ and ISP chooses whether to accept or reject the contract. Note that linear contracts have been shown to be optimal in \cite{Holmstrom1} particularly when agent has a risk averse utility as it is our case in our setting. In fact, if ISP accepts the contract, he chooses an action (a caching effort) $a_i\in A\equiv [0,\infty]$ for each  $CP_i$. ISP rejects the contract if he gets expected utility below a reserve utility denoted by $\overline{H}$. ISP has constant absolute risk aversion (CARA) utility as $H(W)=-e^{-zW}$, where $W$ is wealth and $z>0$ is a fixed constant. CP$_i$ observes a demand, that depends on caching effort $a_i$ by the ISP, and estimates it as a random variable
$D_i:=\log(a_i+1)+\epsilon_i$,  where $\epsilon_i$ is a random error observed for the demand for content of CP$_i$. Each $\epsilon_i $ is assumed to be Gaussian distributed with mean $0$. Random errors are not independent and the covariance matrix $K$ is given by: \[
K =
\left[ {\begin{array}{cc}
	\sigma_1^2 & \rho \sigma_1\sigma_2 \\
	\rho \sigma_1\sigma_2 & \sigma_2^2  \\
	\end{array} } \right].
\]
The total revenue generated for CP$_i$ due to his demand is $X_i=r_iD_i$ where $r_i$ is the revenue per click for $CP_i$ when $D_i$ is, for example, associated to a number of clicks. Each CP$_i$ is assumed to be risk neutral with a utility function expressed as $V_i(X-s_i(X))=X-s_i(X)$. Cost incurred by ISP is assumed to be increasing in the global caching effort as $c(a_1,a_2)=c(a_1+a_2)$.
% Here, caching cost is different for each CP because we assume that each CP provide  different type of contents.
The expected utility of $CP_i$ is given by:
\begin{align*}
E[V(X_i-s_i(X_i))]&=E[V(X_i-(\beta_i X_i))],\\
& =E[X_i(1-\beta_i)]=(1-\beta_i)r_i\log(a_i+1),
\end{align*}
%\begin{eqnarray}\nonumber 
%&E[V(X_i-s_i(X_i))]=E[V(X_i-(\alpha_i+\beta_i X_i))]&\\
%& =E[X_i(1-\beta_i)-\alpha_i] =(1-\beta_i)r_i\log(a_i+1)-\alpha
%_i,&
%\end{eqnarray}
and the expected utility of $ISP$ is given by:
\begin{align*}
E[H(\sum_i[s_i(X_i)-ca_i])]&=E[H(\sum_i[\beta_ir_i(\log(a_i+1)+\epsilon_i)-ca_i])]\\
&=E[-\exp\sum_i[\beta_ir_i(\log(a_i+1)+\epsilon_i)-ca_i]]\\
&=-\exp\{-z\sum_i[\beta_ir_i\log(a_i+1)-ca_i]\\
+\frac{z^2}{2}[(\beta_1r_1\sigma_1)^2+&(\beta_2r_2\sigma_2)^2+2\rho\beta_1\beta_2r_1r_2\sigma_1\sigma_2]\}.
\end{align*}
The expression for the ISP expected utility follows after noting that it is the characteristic function of a Gaussian random vector. ISP's optimization problem is to find an effort level $a_i$ for each CP$_i$ which maximizes its expected utility. Maximizing expected utility over both $a_i$ is equivalent to maximizing its negative exponent term.
%, i.e.,
%$$
%\sum_i[\beta_ir_i\log(a_i+1)-ca_i]-\frac{z}{2}[(\beta_1r_1\sigma_1)^2+(\beta_2r_2\sigma_2)^2+2\rho\beta_1\beta_2r_1r_2\sigma_1\sigma_2]
%$$\\
%\noindent
Therefore, the simplified optimization problem for each $CP_i$, taking into account the ISP optimization problem, is given as the following bilevel optimization problem: 
\begin{align*}
&\hspace{12mm}\max_{a_i, \beta_i} \hspace{2mm} (1-\beta_i)\log(a_i+1)r_i&\\
&\hspace{6mm}\text{s.t.} \hspace{5mm}\sum_i[\beta_ir_i\log(a_i+1)-ca_i]\\
&\hspace{10mm}-\frac{z}{2}[(\beta_1r_1\sigma_1)^2+(\beta_2r_2\sigma_2)^2+2\rho\beta_1\beta_2r_1r_2\sigma_1\sigma_2]\geq \overline{h}\\&
\text{argmax}_{a_1,a_2} \sum_i[\beta_ir_i\log(a_i+1)-ca_i]\\
&\hspace{10mm}-\frac{z}{2}[(\beta_1r_1\sigma_1)^2+(\beta_2r_2\sigma_2)^2+2\rho\beta_1\beta_2r_1r_2\sigma_1\sigma_2]\\
&\hspace{20mm}\text{where} \hspace{1.5mm}\overline{h}=-\log (-\overline{H}).
\end{align*} 
%\begin{eqnarray}
%\nonumber&\max_{a_i, \alpha_i,\beta_i} \hspace{2mm} (1-\beta_i)\log(a+1)r_i-\alpha_i&\\\nonumber \noindent
%&\text{s.t.}\sum_i[\beta_ir_i\log(a_i+1)-ca_i]\\
%&-\frac{z}{2}[(\beta_1r_1\sigma_1)^2+(\beta_2r_2\sigma_2)^2+2\rho\beta_1\beta_2r_1r_2\sigma_1\sigma_2]\geq \overline{h}&\\ \nonumber
%&\text{argmax}_{a_1,a_2} \sum_i[\beta_ir_i\log(a_i+1)-ca_i]-\frac{z}{2}[(\beta_1r_1\sigma_1)^2+(\beta_2r_2\sigma_2)^2+2\rho\beta_1\beta_2r_1r_2\sigma_1\sigma_2]&\\ \nonumber \noindent
%&\text{where} \hspace{1.5mm}\overline{h}=-\log (-\overline{H})&
%\end{eqnarray}
The lower-level optimization problem, i.e. the ISP effort optimization problem, as the following solution depending on contracts proposed by both CPs.
\begin{lemma}
	The optimal ISP effort level $a_i^*$ for each CP$_i$ is given by
	$$a_i^*=\max\left(\frac{\beta_ir_i}{c}-1,0\right); i=1,2$$
\end{lemma}
%\begin{lemma}
%	There exist continuum of equilibrium $(\beta_1^*,\beta_2^*)$ of the game between CPs satisfying following equality:
%	\begin{align*}
%	&\hspace{2cm}\sum_i[\beta_i^*r_i\log\left(\frac{\beta_i^*r_i}{c}\right)-\beta_i^*r_i]\\
%	&-\frac{z}{2}[(\beta_1^*r_1\sigma_1)^2+(\beta_2^*r_2\sigma_2)^2+2\rho\beta_1^*\beta_2^*r_1r_2\sigma_1\sigma_2]=\overline{h}
%	\end{align*}
	
%\end{lemma}
An important assumption is that the ISP will accept the CP$_i$ contract if and only if his expected net utility $E(s_i(X_i)-ca_i)$ obtained from CP$_i$ is positive. Hence, if $\sum_i[s_i(X_i)-ca_i]) \geq 0$, the ISP will accept both contracts. Considering this natural case (other case is not of interest here as there is only one CP and then no game between several CPs), yields that for all risk averse parameter $z$, the ISP utility $H(W)\geq -1$ and a natural minimum expected utility is $\overline{H}:=-1$. 

%Then, under this assumption on the minimum expected utility level, the ISP will accept both contracts and there exists a unique equilibrium for the non-cooperative game between CP. This game is studied in the following section.


%Now, $-1 \leq \overline{H}\leq 0$ i.e.,   $0\leq \overline{h}<\infty$, and for $\overline{H}>-1 (\overline{h}>0)$, there could exist continuum of equilibrium of the game between CPs s.t. participation constraint is satisfied at equality. For the uniqueness of the equilibrium we need to assume that $\overline{H}=-1 (\overline{h}=0)$, as under this assumption participation constraint will always be satisfied. The uniqueness of the equilibrium of the non-cooperative game between CPs (at upper level) will allow us to compare the neutral and non-nuetral regime. Non-neutral being the one where ISP is allowed to chooses different caching decision $(a_i)$ for each CP$_i$ and neutral being the case where ISP is restricted to take same caching decision $(a_1=a_2=a)$ for each CP. 


%$r_1/r_2$, $\rho$ and $c$ on Social Utility when ISP applies common and separate efforts for CP respectively. We set parameters $r_1=20$, $P_1=P2=1$, $\sigma_1=\sigma_2=0.25$ and $\overline{H}=200$. We set $c_1=c_2=c/2$, in Fig.~\ref{fig:Utility1}, $r_2=15$ in Fig.~\ref{fig:Utility2} and $c_1=1.5$ and $c_2=1$. in Fig.~\ref{fig:Utility3}.
%Maximizng expected utility over $a$ given is equivalent to maximizing following\\
%$
%\alpha_1+\alpha_2+(\beta_1r_1P_1+\beta_2r_2P_2)a-\frac{ca^2}{2}-\frac{r}{2}((\beta_1r_1P_1\sigma_1)^2+(\beta_2r_2P_2\sigma_2)^2+2\rho\beta_1\beta_2r_1P_1r_2P_2\sigma_1\sigma_2)
%$\\
%Now, each CP solves his maximization problem subject to common constraints and $CP_i$ solves:
%Proposition 3 gives equilibrium behavior of CPs and ISP. Here also $\beta_i^*$ takes unique value at equilibrium and CPs set $\alpha_i^*\text{s}$ in such a way that they extract all the surplus from ISP and ISP will only get his reserve utility. There is continuum of equilibria for this game. ISP does not differentiate between CPs. $\beta_i^*$ is increasing in $r_iP_i$. Also, decreasing in $r_jP_j$ for $\rho>0$ and is increasing in $r_jP_j$ for $\rho<0$ (similar to seperate effort case). The benefit by effort of ISP is shared, however, an increase in $r_iP_i$ increases the marginal benefit of $CP_i$ from the effort exerted by the ISP. 

% \begin{figure}[h!]
%	\begin{center}
%		\includegraphics[scale=0.5]{figures/Fig2.png}
%		\caption{\textit{Effect of disparity between revenue per click rates of CPs on Social Utility.}. }
%	\end{center}
%	\label{fig:figure2 }
%\end{figure}

 
% \begin{figure}[h!]
%	\begin{center}
%		\includegraphics[scale=0.5]{figures/Fig3.png}
%		\caption{\textit{Effect of correlation coefficient on Social Utility.}We set parameters $c_1=c_2=c/2$, $r_1=20$,$r_2=15$ $P_1=P2=1$, $\sigma_1=\sigma_2=0.25$, and $\overline{H}=200$. }
%	\end{center}
%	\label{fig:figure2 }
%\end{figure}


%From figure 2, it can be seen that as the difference between $r_1$ and $r_2$ is higher, disparity is higher in case of seperate Effort. Clearly it implies that seperate effort increases asymmetry in the between CPs in the network.


%Expected Utility of $CP_i$ at equilibrium:
%
%$$
%E[V_i]=(1-\beta_i^*)r_iP_ia^*-\alpha_i^*=(1-\beta_i^*)r_iP_i\frac{\beta_1^*r_1P_1+\beta_2^*r_2P_2}{c}^*-\alpha_i^*$$
%=(1-\frac{(1+rc\sigma_2^2)-(\frac{r_2P_2}{r_1P_1})rc\rho \sigma_1 \sigma_2}{(1+rc\sigma_1^2)(1+rc\sigma_2^2)-\rho^2 r^2 c^2 \sigma_1^2 \sigma_2^2})r_iP_i\frac{r_1P_1[1+rc(\sigma_2^2-\rho\sigma_1\sigma_2)]+r_2P_2[1+rc(\sigma_1^2-\rho\sigma_1\sigma_2)]}{(1+rc\sigma_1^2)(1+rc\sigma_2^2)-\rho^2 r^2 c^2 \sigma_1^2 \sigma_2^2}-\alpha_1

%\section{Forcing neutral behavior}
%Competition between CPs induces non-neutral behavior in separate effort case, i.e. different effort made by the ISP for each CP ($a_1 \neq a_2$). In this case, neutrality can be imposed by making the same effort of the ISP for both CPs equal. We can think about an external control done by an entity (the governmental authority for example). This external entity may impose a tax on the contents such that the resulting investment strategy of the ISP is neutral, i.e. $a^*_1=a^*_2$. We can then think about a three layers hierarchical game where:
%\begin{enumerate}
%	\item At the higher level (authority level), the authority determines the taxes that each CP has to pay on their benefit (for example a percentage of the net profit) in order to minimize the difference between $a_1^*$ and $a_2^*$.
%	\item At the intermediate level, based on this tax, each CP $i$ determines the optimal contract $S_i(.)$ with the ISP.
%	\item Finally, at the lower level, the ISP determines optimally his investment $a_i$ for each CP $i$ traffic.
%\end{enumerate}
%When the tax $t_i$ is imposed on the revenue generated by $CP_i$, new revenue becomes $(1-t_i)X_i$.\\
%Equilibrium Solution for new $X_i$:
%$$
%a_1^*=\frac{r_1P_1(1-t_1)(1+rcA)-r_2P_2(1-t_2)rcA}{c[1+2rcA]}
%$$
%$$
%a_2^*=\frac{r_2P_2(1-t_2)(1+rcA)-r_1P_1(1-t_1)rcA}{c[1+2rcA]}
%$$
%$$
%\beta_1^*=\frac{c(a_1^*+a_2^*)}{r_1P_1(1-t_1)}, \beta_2=\frac{c(a_1^*+a_2^*)}{r_2P_2(1-t_2)}
%$$
%$$
%\beta_1^*=\frac{r_1P_1(1-t_1)+r_2P_2(1-t_2)}{r_1P_1(1-t_1)[1+2rcA]}
%$$
%$$
%\beta_2^*=\frac{r_1P_1(1-t_1)+r_2P_2(1-t_2)}{r_2P_2(1-t_2)[1+2rcA]}
%$$\\
%where $A=\sigma_1^2+\sigma_2^2+2\rho\sigma_1\sigma_2$.\\
%To make $a_1^*=a_2^*$, taxes imposed should be according to following equation:
%$$
%\frac{1-t_1}{1-t_2}=\frac{r_2P_2}{r_1P_1\label{den}}
%$$
%(this comes from equating the expressions obtained form $a_1^*$ and $a_2^*$)
%
%\begin{figure}[h!]
%	\begin{center}
%		\includegraphics[scale=0.35]{figures/fig3levels.pdf}
%		\caption{Global interaction system between authority, content providers and the service provider.}
%	\end{center}
%	\label{fig:figure2 }
%\end{figure}


==> model.tex <==
 The ISP is risk-averse
and chooses, for each CP $i$, an effort level $a_i$ that benefits the CP$_i$ under the contract. ISP will accept the contract with CP$_i$ only if it gets at least reserve utility denoted $\overline{H}$. CPs observe only a noisy
signal of the effort level chosen by the ISP. Let $X_i$ denote the revenue generated by CP$_i$ and $s_i(X_i)$ denote the share of $X_i$ that goes to the ISP under the contract.  Let $V_i(\cdot)\in\mathbb{R}_+$ denotes the utility associated to the revenue generated by CP$_i$ and it is a function of the net revenue of the CP$_i$, i.e., $X_i -s(X_i)$. This function $V_i(.)$ is typically increasing concave function.The utility of the ISP is a function $H(s_1(X_1),s_2(X_2), a_1,a_2)\in\mathbb{R}_+$. We assume that this function is increasing in $s_i(X_i)$ and decreasing in $a_i$.
%In this section, we analyze a game between two CPs which offer contract to common ISP, under which ISP chooses an effort level $a$ that benefits both CPs. ISP is risk averse and will accept the contract only if it gets at least reserve utility say $\overline{H}$.  
% Let $V_i(\cdot)\in\mathbb{R}_+$ denotes the utility associated to the revenue generated by $CP_i$. For each $X_1$, $X_2$, $s_1(X_1)$, $s_2(X_2)$ and $a$, $H(s_1(X_1),s_2(X_2),a)\in\mathbb{R}_+$ denote the utility of the ISP. We assume that $H(\cdot)$ is increasing in $s_i(X_i)$ and decreasing in $a$.
%$$\frac{\partial H(s_1(X_1),s_2(X_2),a)}{\partial s_i(X_i)}>0, $$
%$$\frac{\partial H}{\partial a_i}(s_1(X_1),s_2(X_2),a)<0. $$

 We further assume that $H(s_1(X_1),s_2(X_2),a_1,a_2)=U(s_1(X_1),s_2(X_2))-C(a_1,a_2)$, where $U(s_1(X_1),s_2(X_2))$ is the utility of the ISP from the total revenues shared from the CPs and $C(a_1,a_2)$ is the cost incurred for applying the efforts $a_1$ and $a_2$. %As the ISP is generally assumed to be risk averse, then $U(\cdot)$ is strictly concave in both terms.
 
Each $CP$ aims at determining an optimal sharing function (contract) $s_i(.)$ that maximizes its expected net revenue. The optimization problem associated to CP$_i, i=1,2$ is given by the following constraint optimization problem:
\begin{eqnarray} \nonumber
&\max_{a_1,a_2, s_i(\cdot)}E_{X_i}[V_i(X_i-s_i(X_i))]&\\
&\text{ s.t } \hspace{3.5mm} E_{X_1,\;X_2}[H(s_1(X_1),s_2(X_2),a_1,a_2)]\geq \overline{H}&\\ 
&\max_{a_1,a_2}E_{X_1,\;X_2}[H(s_1(X_1),s_2(X_2),a_1,a_2)]. &
\end{eqnarray}
Constraint $(1)$ guarantees to the ISP the minimum expected utility $\overline{H}$ and is called as individual rationality (IR) or the participation constraint. The second constraint is the ISP's  optimization problem and is called as incentive compatibility constraint (IC). It also captures the fact that the CPs cannot observe effort level of the ISP. The structure of the optimization problem is hierarchical and can be studied considering a Stackelberg solution concept. In fact, the principal (here each CP) can be seen as a leader and the agent (here the ISP) as the follower who plays after observing the action of the principal. But in our setting, there is another level of complexity as there are two principals and therefore, it  gives a static game between CPs with shared constraints. Then, the use of generalized Nash Equilibrium Point (GNEP)\cite{GNEP} can be useful in order to analyze the optimal sharing contracts at the principal level considering the agent's action.  It is in general hard to solve this type of complex game for arbitrary sharing function. 

In the following we focus on the linear sharing functions (or contracts). We first consider the case where the ISP differentiates the CPs and puts separate for each of them and then consider the case where the CPs are not differentiated and the ISP puts common efforts for both the CPs. Our former case corresponds to the non-neutral regime and the later to the neutral regime.\\


 

%Let $X_i$ as a random variable with a distribution $F(X_i,a)$, parameterized by the ISP's action with density function $f(X_i,a_i)$ and well defined $f_{a}$ and $f_{aa}$ for all $(X_i,a)$. Also, let $g(X_1,X_2,a)$ be joint density function with well defined $g_{a}$ and $g_{aa}$.
%\\The expected utility of $CP_i$ is given by
%\begin{eqnarray}
%&E_{X_i}[V(X_i-s_i(X_i))]=\int V(X_i-s(X_i))f(X_i,a)dX_i&
%%&=a_i-\int s(X_i)f(X_i,a_i)dX_i&
%\end{eqnarray}
%The expected utility of $ISP$ is given by
%\begin{eqnarray}\nonumber
%&E_{X_1, X_2}[U(\sum_is_i(X_i))-C(a)]&\\
%=\int\int U(\sum_is_i(X_i))g(X_1,X_2,a)dX_1dX_2 - C(a)&
%\end{eqnarray}
%Then we have\\
%For $CP_1$:
%\begin{eqnarray}\nonumber
%&\max_{s_1(X_1)} \hspace{3mm} \int V(X_1-s_1(X_1))f(X_1,a)dX_1&\\\nonumber
%&\text{ s.t } \int \int U(s_1(X_1)+s_2(X_2))g(X_1,X_2,a)dX_1dX_2 - C(a)\geq \overline{H}&\\\nonumber
%&\max_{a}  \int \int U(s_1(X_1)+s_2(X_2))g(X_1,X_2,a)dX_1dX_2 - C(a)&
%\end{eqnarray}
%For $CP_2$:
%\begin{eqnarray}\nonumber
%&\max_{s_2(X_2)}\hspace{3mm}\int V(X_2-s_2(X_2))f(X_2,a_2)dX_2&\\\nonumber
%&\text{ s.t }\int \int U(s_1(X_1)+s_2(X_2))g(X_1,X_2,a)dX_1dX_2 - C(a)\geq \overline{H}&\\\nonumber
%&\max_{a} \int \int U(s_1(X_1)+s_2(X_2))g(X_1,X_2,a)dX_1dX_2 - C(a)&
%\end{eqnarray}
%
%This is a game between $CP_1$ and $CP_2$ having shared constraints. Such a game is called as GNEP.
%Contracts are linear type.

==> symmetric.tex <==
In this section, we consider the special case where CPs are symmetric in terms of their monetization power , i.e., $(r_1=r_2=r)$ and compare the utilities of CPs and ISP in non-neutral and neutral regimes. The following corollary to Thm.~\ref{Thm:NN-asy} gives the equilibrium contracts in the non-neutral regime.
%\subsection{Non-Neutral regime}
%In this section, we consider that ISP is allowed to make different investment $a_i$ for each CP$_i ; i=1,2$. The problem for each $CP_i$ reduces to 
%\begin{align*}
%&\hspace{8.9mm}\max_{a_1, a_2 \beta_i} \hspace{3mm} (1-\beta_i)r\log(a_i+1)\\
%&\text{s.t.}\\
%&\text{argmax}_{a_1,a_2}\hspace{3mm} \sum_iz\left(\beta_ir\log(a_i+1)-ca_i\right)
%\end{align*}
%%\begin{eqnarray}
%%\nonumber&\max_{a_i, \beta_i} \hspace{2mm} (1-\beta_i)\log(a+1)r&\\\nonumber \noindent
%%&\max_{a_1,a_2}\hspace{3mm} \sum_iz\left(\beta_ir\log(a_i+1)-ca_i\right)&\\
%%\end{eqnarray}
%Following Lemma gives the equilibrium solution 
\begin{corollary} \label{lma:NN-sym}
	In the non-neutral regime equilibrium contract is given by 
	\begin{equation}
	\beta_1^{NN}=\beta_2^{NN}=\begin{cases}
	0  &\mbox{  if }  \frac{r}{c}\leq 1, \\
	\frac{1}{W\left(\frac{r}{c}e\right)}  &\mbox{  if }  \frac{r}{c} > 1,
	\end{cases}
	\end{equation}
	where $W(\cdot)$ is the Lambertw function. Further, the effort levels of the ISP for are given by
	\begin{equation} \label{eqn:NN-a}
a_i^{NN}=a^{NN}=\max\left(\frac{\beta^{NN} r}{c}-1,0\right) \hspace{1.5mm} \forall i=1,2.
\end{equation}
\end{corollary}
%\begin{lemma} \label{lma:NN-sym}
%	The investment decision	of ISP for each CP$_i; i=1,2$ is given by
%	\begin{equation} \label{eqn:NN-a}
%	a_i^{NN}=a^{NN}=\max\left(\frac{\beta^{NN} r}{c}-1,0\right) \hspace{1.5mm} \forall i=1,2
%	\end{equation}
%	and the share proportion for both CPs are equal and is given by:	
%\begin{equation}
%\beta_i^{NN}=\beta^{NN}=\begin{cases}
%0  &\mbox{  if }  \frac{r}{c}\leq 1, \\
%\frac{1}{W\left(\frac{r}{c}e\right)}  &\mbox{  if }  \frac{r}{c} > 1
%\end{cases}
%\end{equation}
%where $W(\cdot)$ is the Lambertw function.
%%	\begin{equation}
%%	\beta_i^{NN}=\beta^{NN}=\frac{1}{W\left(\frac{r}{c}e\right)} \hspace{2mm} \forall \hspace{1mm}  \frac{r}{c}>1
%%	\end{equation}
%%		\begin{equation}
%%	\beta_i^{NN}=\beta^{NN}=0\hspace{2mm} \forall \hspace{1mm}  \frac{r}{c}\le 1
%%	\end{equation}
%\end{lemma}

Now, utility of each $\CPi,i=1,2$ at equilibrium is given by
\begin{eqnarray}\nonumber
\UCPi=(1-\beta^{NN}) r\log(a^{NN}+1)=\frac{(1-\beta^{NN})^2}{\beta^{NN}}r,
\end{eqnarray}
and utility of the ISP at equilibrium is give by:
\begin{eqnarray}\nonumber
&\UISP=\left[2\beta^{NN} r \
\log(a^{NN}+1)-c(2a^{NN})\right]&\\
&=\left[2(r+c)-4\beta^{NN}r\right].
\end{eqnarray}

%%
%\subsection{Neutral regime}
%In this section, we consider that ISP is allowed to make different investment $a_i$ for each CP$_i ; i=1,2$. The problem for each $CP_i$ reduces to 
%\begin{align*}
%&\hspace{8mm}\max_{a, \beta_i} \hspace{2mm} (1-\beta_i)\log(a+1)r\\
%&\text{s.t.}\\
%&\text{argmax}_{a}\hspace{3mm} z\left(\sum_i\beta_ir\log(a+1)-2ca\right)
%\end{align*}
%
%%\begin{eqnarray}
%%\nonumber&\max_{a, \beta_i} \hspace{2mm} (1-\beta_i)\log(a+1)r&\\\nonumber \noindent
%%&\text{s.t.}&\\\nonumber
%%&\text{argmax}_{a}\hspace{3mm} \sum_iz\left(\beta_ir\log(a+1)-2ca\right)&\\
%%\end{eqnarray}
The following corollary to Thm.~\ref{Thm:Neutral-asym} specializes the results in the neutral regime.
\begin{lemma} \label{lma:N-sym}
	The equlibrium contracts in the neutral regime is given by:	
\begin{equation}
\beta_i^{N}=\beta^{N}=\begin{cases}
0  &\mbox{  if }  \frac{r}{2c}\leq 1, \\
\frac{1}{2W\left(\frac{r}{2c}e^{0.5}\right)}  &\mbox{  if }  \frac{r}{2c} > 1
\end{cases}
\end{equation}
and the common effort level by the ISP is given by
\begin{equation} \label{eqn:N-a}
a^{N}=\frac{\beta^{N} r}{c}-1
\end{equation} 
%	\begin{equation}
%	\beta^{N}=\frac{1}{2W\left(\frac{r}{2c}e^{0.5}\right)}
%	\end{equation}
\end{lemma}
Utility of each CP at equilibrium is then 
\begin{eqnarray}\nonumber
(1-\beta^{N}) r\log(a^{N}+1)
=\frac{(1-\beta^{N})^2}{2\beta^{N}}r
\end{eqnarray}
and the ISP utility is:
\begin{eqnarray}\nonumber
\left[2\beta^{N} r \log(a^{N}+1)-2c(a^{N})\right]=\left[r+2c-3\beta^{N}r\right].
\end{eqnarray}  \subsection{Comparison between Non-neutral and neutral regime}
In this section we study the comparison between Non-neutral and neutral regime when CPs are symmetric and have same revenue per click rates.

%\begin{figure*}[!tb]
%	\centering
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig1}%
%		\label{fig:effort}}
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig2}%
%		\label{fig:beta}}
%		\hspace{0.55cm}
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig3}%
%		\label{fig:beta}}
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig4}%
%		\label{fig:Utility1}}
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig5}%
%		\label{fig:Utility2}}
%	%		\subfloat[]{\includegraphics[scale=0.04]{figures/Gain3}%
%	%		\label{fig:Gain4}}
%	\caption {Comparison between Non-neutral and neutral w.r.t c}
%	\label{fig:Gain}
%\end{figure*}
%
%\begin{figure*}[!tb]
%	\centering
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig2a}%
%		\label{fig:effort}}
%		\subfloat[]{\includegraphics[scale=0.4]{figures/Fig2e}%
%		\label{fig:beta}}
%	\hspace{0.55cm}
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig2b}%
%		\label{fig:Utility1}}
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig2c}%
%		\label{fig:Utility2}}
%	\subfloat[]{\includegraphics[scale=0.4]{figures/Fig2d}%
%		\label{fig:Utility2}}
%	
%	\caption {Comparison between Non-neutral and neutral w.r.t $r$}
%	\label{fig:Gain}
%\end{figure*} 

\begin{lemma} \label{lma:betacomp}
Proportion of revenue shared by each CP in higher in non-neutral regime as compared to that in neutral regime, i.e.,	$$\beta^{NN} \geq {\beta^{N}}$$
\end{lemma}
Above lemma suggest that CPs share more revenue in non-neutral regime as compared to neutral regime.

\begin{lemma} \label{lma:effortcomp}
	ISP makes more investment in higher in non-neutral regime as compared to that in neutral regime, i.e.,	$$a^{NN} \geq {a^{N}}$$
\end{lemma} 

Proof of above lemma follows directly. Since, investment decision by ISP is monotonically increasing in shared revenue proportion (from eqns. (\ref{eqn:NN-a}) and (\ref{eqn:N-a})), by lemma \ref{lma:betacomp} it is clear that ISP  make more investment in non-neutral regime as compared to neutral regime.

\begin{lemma} \label{lma:UISPcomp}
	Utility of ISP is higher in non-neutral regime as compared to that in neutral regime.
\end{lemma}

\begin{lemma} \label{lma:UCPcomp}
	Utility of each CP is higher in non-neutral regime as compared to that in neutral regime.
\end{lemma}
